Certified private data release for sparse Lipschitz functions

As machine learning has become more relevant for everyday applications, a natural requirement is the protection of the privacy of the training data. When the relevant learning questions are unknown in advance, or hyper-parameter tuning plays a central role, one solution is to release a differentially private synthetic data set that leads to similar conclusions as the original training data. In this work, we introduce an algorithm that enjoys fast rates for the utility loss for sparse Lipschitz queries. Furthermore, we show how to obtain a certificate for the utility loss for a large class of algorithms.

==> Workshop/Section1_intro.tex <==

\vspace{-0.5in}
\begin{abstract}
Differential privacy is the de facto standard for protecting privacy in a variety of applications. One key challenge is private data release, which is particularly relevant in scenarios where limited information about the final application is available in advance. In this context, strong theoretical utility guarantees provide confidence that insights derived from the released dataset agree with the actual underlying data. In this work, we i) introduce an algorithm that enjoys fast rates for the utility loss for sparse Lipschitz queries and ii) provide a way to compute a certificate for the maximum utility loss  for a large class of algorithms.
%and present numerical simulations for real world data sets demonstrating its power. 
%experimental evidence fo
%are required, or to $n^{-1/(s+1)}$ when the data lies on an unknown s-dimensional subspace, disregarding logarithmic factors. We therefore obtain practically meaningful rates for moderate constants $s$ which motivates future work on computationally efficient approximate algorithms for this~problem.
\end{abstract}
% \begin{keywords}%
% Differential Privacy, Data Sanitization, Private Data Release\end{keywords}


\section{Introduction}
% \let\thefootnote\relax\footnotetext{$^*$ Equal contribution; email address  konstantin.donhauser@ai.ethz.ch}
% As sensitive personal information continues to be extensively used in modern data analysis, ensuring the privacy of individual data points has become an increasingly critical necessity.
% Differential privacy
% (DP)~\citep{dwork2006calibrating} 
% is used by  
% %has grown to become the de-facto
% %standard for privacy protection 
% both governmental agencies \citep{Census} and commercial actors \citep{industry_eps}.
% Intuitively, differential privacy ensures that no individual data point has a
% significant impact on the algorithm's output. This obscures whether a particular sample is part of the data set or not. More formally, a probabilistic algorithm $\mathcal{A}$ is said to be $\epsilon$-DP 
% if it satisfies the conditions in
% Definition~\ref{eq:defdp}. 

% \begin{definition}
% \label{eq:defdp}
%     An algorithm $\gA$ is $\epsilon$-DP with $\epsilon>0$ if for any datasets $D, D'$ differing in a single entry and any measurable subset $S \subset \mathrm{im}(\mathcal A)$ of the image of $\mathcal A$, we have
%     %\footnote{Commonly a slightly more general notion of DP is used where the algorithm $\mathcal A$ takes the dataset $D$ as input and therefore may also be sensitive to permutations of the dataset.}
% $\f{\P}{\f{\gA}{D}\in S} \leq \exp\brace{\epsilon} \f{\P}{\f{\gA}{D'}\in S}$
% % + \delta$

% where $\mu_D$ is the empirical measure of $D$.
Several works focus on preserving differential privacy while extracting specific information from data,
%completing specific, a-priori known tasks on data, 
such as executing specific machine learning algorithms~\citep{bassily2014private,chaudhuri2011differentially,feldman2014sample,raskhodnikova2008can}
or answering a number of predetermined queries~\citep{blum2005practical,dagan2022bounded,dwork2004privacy,ghazi21union,hardt2010geometry,steinke2016between}.
However, a major shortcoming of these methods is that any analysis can only be performed once without further loosening privacy guarantees.
%the statistics must be known a priori as further queries can on only be answered by sacrificing privacy guarantees (i.e., by increasing $\epsilon$). 
An approach that mitigates this shortcoming is to release a synthetic dataset in a differentially private manner that is ideally representative of the original data. This process is also known as ``data sanitization"~\citep{dwork2009complexity} and has the advantage that any operation performed on the released dataset will not introduce further privacy leakage
- a particularly useful property when it is difficult to predict potential future use cases.
%and data sanitization thus overcomes the shortcomings of previously mentioned approaches. Furthermore, data sanitization techniques become particularly compelling when the aim is to make the data accessible to a diverse set of users or when it is difficult to predict potential future use cases accurately.
% or when the statistics of interest may change over time. 
% In many practical applications only limited information about the statistics of interest  is available when 

When designing data sanitization algorithms, the "representativeness" of the synthetic dataset is 
usually measured in terms of the utility loss over 
a broad function class \citep{blum2013learning,mwem,liu2021iterative}.
%objective is  usually to attain a small utility loss over a broad  function class \citep{blum2013learning,mwem,liu2021iterative}. 
%Instead, another line of work aims to preserve differential privacy for a-priori unknown queries from a 
%that is differentially private with respect to a whole set of queries.
%However, in many situations, different users may like to use a dataset 
%request different statistics from the data and anticipating the needs of all potential users in advance can often be very challenging; this is for instance the case for census data~\citep{Census}. To address this shortcoming, a common solution is to release a differentially private, synthetic data set. 
%This approach, also known as ``data sanitization"~\citep{dwork2009complexity}, provides guarantees over a class of queries, denoted as $\mathcal F$. F
Formally, if an algorithm $\mathcal A$ takes an empirical distribution $\mu_D$ of a data set $D$  as input and returns a probability measure $\mathcal A(D)$, we define the utility loss as \footnote{We note that in the literature, the algorithm's output $\mathcal A(D)$ is usually a dataset rather than a probability measure. Nevertheless, a dataset can always be constructed from a probability measure using standard techniques such as subsampling or discretization (see e.g., \citep{boedihardjo2022private,Yiyun23}). We therefore simplify our notation by disregarding this distinction in our paper. }
%Specifically, the algorithm should have a low utility loss when applied to the predetermined class of functions or queries $\mathcal F$:
\begin{equation}
\label{eq:utilityloss}
    \utilityloss(\mu_D, \mathcal A(D) ) := \sup_{f\in \mathcal F} \left\vert \int f(x) d\mu_D - \int  f(z) d\algoD \right\vert.
\end{equation}

A large body of research empirically demonstrates that data sanitization algorithms perform well over various important types of queries; specifically, previous works have studied obtaining certain predefined statistics or training specific machine learning models  \citep{aydore2021differentially,gaboardi2014dual,mwem,jordon2019pate,liu2021iterative, mckenna2021winning, mckenna2022aim, mckenna2019graphical, vietri2022private}.  However, in the context of differentially private data release, assessing the quality in a DP way of the synthetic data set poses a fundamental problem. %Indeed, publicly  releasing the utility loss~\eqref{eq:utilityloss} between $\mu_D$ and $\algoD$ might leak information about $\mu_D$, violating privacy guarantees.
% While some algorithms address this issue by providing tight bounds for the non-asymptotic decay rate of the utility loss (see   Section~\ref{sec:relatedwork} for related works), the need for actual numerical guarantees arises in numerous real-world applications.
We address this short-coming by releasing, together with the synthetic data, a certificate for the utility loss; that is a upper bound for the utility loss that can be computed for any (finite) measure $\algoD$ and holds with high-probability uniformly for all measures. Unlike finite sample guarantees, which are often only tight in the limit as the amount of data samples goes to infinity,  the certificate proposed in this paper yields practically meaningful tight guarantees for the specific application.

We are first to study  the case where $\mathcal F$  is the set of all $s$-sparse $1$-Lipschitz functions (i.e. functions that only vary in $s$-dimensions of the input). 
Queries in this function naturally arise when investigating the relationship between (a few) features. For instance, census data \citep{Census} might be used to understand the relationship between gender, income and job category. Posing this type of restrictions on the number of predictive features is common for machine learning applications, either through explicit feature selection or sparsity-inducing loss functions. %Moreover, such statistics can often be approximated using sparse, Lipschitz functions. For example, any $s$-moment $f(x) = \frac{1}{\vert S\vert} \prod_{i \in S} x_{i}$ with
% $\vert S \vert \leq s$ is contained in $\mathcal F$. 
Moreover  guarantees for sparse Lipschitz functions also extend beyond preserving sparse marginals; they maintain the clustering structure on the projected subspaces, and more generally guarantee a small $1$-Wasserstein distance over all $s$-sparse marginal measures (by the  Kantorovich-Rubinstein Duality Theorem \citep{Villani2008OptimalTO})
%of two measures...? \fy{gotta make sure they don't mistake s sparse marginal and s-way marginal}
\begin{equation}
\label{eq:wassersteinsparse}\utilityloss(\mu_D, \algoD ) =  \sup_{S \subset \{1, \cdots, d\}; \vert S \vert =s} W_1 \left(P_{\#}^{S}\mu_{D},  P_{\#}^{S}\algoD\right),
\end{equation}
where $W_1$ is the $1$-Wasserstein distance, and $P_{\#}^{S} \mu_{D}$ is the marginal measure of $\mu_D$ on
the $s$-dimensional subspace defined by the coordinates in $S$. 




%Specifically, we consider the function class $\mathcal F$ consisting of all $s$-sparse $1$-Lipschitz functions (i.e. functions that only vary in $s$-dimensions of the input). 
%As we argue, one common use of many data sets is to investigate the relationship between (a few) features. For instance, census data \citep{Census} might be used to understand the relationship between gender, income and job category. Such statistics are naturally sparse functions and can often be approximated using sparse,Lipschitz functions.
%Moreover, in machine learning applications it is common to restrict the number of relevant features through explicit feature selection or sparsity-inducing loss functions.
%Furthermore, any $s$-way marginal frequency $f(x) = \frac{1}{\vert S\vert} \prod_{i \in S} x_{i}$ with $\vert S \vert \leq s$ is contained in $\mathcal F$. 
%Furthermore, 
% Indeed, by the Kantorovich-Rubinstein Duality Theorem \citep{Villani2008OptimalTO}, the utility loss \eqref{eq:utilityloss} is equal to the maximum $1$-Wasserstein distance over all $s$-sparse marginal measures:
%\begin{equation}
%\label{eq:wassersteinsparse}\utilityloss(\mu_D, \algoD ) =  \sup_{S \subset \{1, \cdots, d\}; \vert S \vert =s} W_1 \left(\mu_{D}^{S}, \algoD^S\right),
%\end{equation}
%where  $W_1$ is the $1$-Wasserstein distance, and $\mu_{D}^{S}$ the marginal measure of $\mu_D$ on the $s$-dimensional subspace defined by the coordinates in $S$. 

%; this is an important problem that has been extensively studied in the privacy literature (see Section~\ref{sec:relatedwork})


\subsection{Contributions} In this work, we are first to propose a sample-efficient DP algorithm that simultaneously returns a synthetic data set that achieves a small utility loss for $s$-sparse Lipschitz functions and furthermore returns a certificate  on its maximum utility loss.  In particular, 


    
\paragraph{Algorithm} we derive in Section~\ref{sec:algo} a differentiable private and computable high-probability certificate  on the utility loss that can inform the practitioner about the quality of the synthetic data set. Algorithm~\ref{alg:mainalgo} then outputs a DP measure by minimizing the upper bound in the certificate. 
    % To the best of our knowledge, releasing a certificate along with synthetic data is a novel approach in the literature. 

\paragraph{Theoretical analysis} we show in Appendix~\ref{sec:mainthm} that the $\epsilon$-DP  measure released by Algorithm~\ref{alg:mainalgo} has an optimal exponential dependency in the non-asymptotic decay rate for the utility loss of $1/s$. More precisely, when the underlying space is the $d$-dimensional hypercube $T = [0,1]^d$ equipped with the $\ell_\infty$-metric, we show in Theorem~\ref{cor:rates} the following upper bound on the expected utility loss
\begin{equation}
    \mathbb E ~\utilityloss (\mu_D, \algoD) \lesssim_s  ~d \left( \frac{ \log^2(\epsilon n)}{n \epsilon}\right)^{1/s}.
\end{equation}
We extend previous works \citep{boedihardjo2022private,Yiyun23} which studied the case where $\mathcal F$ is the set of all Lipschitz continuous functions ($s=d$). As we show, restricting $\mathcal F$ to $s$-sparse functions allows us to effectively overcome the curse of dimensionality.  

% instead of $1/d$. Thus, we show that we can effectively address the curse of dimensionality (see Equation~\eqref{eq:ubfull} in Section~\ref{sec:relatedwork}) by restricting $\mathcal F$ to 





 \begin{figure}[t!]

%\vspace{-0.2in}
    \centering
    \begin{subfigure}{\textwidth}
        \centering
\includegraphics[width=\textwidth]{figures/legend_bench.png}
        % No caption for the first plot
    \end{subfigure}
    \hspace{0.05\textwidth}
    \begin{subfigure}{0.33\textwidth}
\includegraphics[width=\textwidth]{figures/ACSIncomeCAAL_fig1.png}
             \caption{Income AL 18'}
         \label{fig:intro1}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \centering
\includegraphics[width=\textwidth]{figures/TravelTimeNYMA_fig1.png}
             \caption{TravelTime MA 18'
            }
         \label{fig:intro2}
        \end{subfigure}~
    \caption{\small 
    Upper and lower bound of the utility loss (see Appendix~\ref{apx:experiments}) and the utility loss of the empirical measure of the 'raw" public data as a function of 
    function of the discretization parameter $k$   (dashed horizontal line). 
    Moreover, the upper bound from Equation~\eqref{eq:pluginub} with $\delta=0.1$ for Algorithm~\ref{alg:mainalgo} (blue line). 
}     
    \label{fig:intro}
\end{figure}



\paragraph{Numerical simulations}
we illustrate the certificate (blue line) and the utility loss (yellow line) for two real world data sets in Figure~\ref{fig:intro} as a function of a discretization parameter $k$.   To improve the run-time complexity, we use an efficient approximate version of Algorithm~\ref{alg:mainalgo} based on public data. We additionally plot the utility loss of the "raw" public data against the private data (horizontal black  line). 
We can clearly observe that i) the certificate gives a tight upper bound for the actual utility loss and ii) the synthetic data set achieves a significantly smaller utility loss than the "raw" public data. We present  more extensive experiments in Appendix~\ref{sec:publi_data}.







%As we argue, sparse $1$-Lipschitz continuous functions still pose an important class of functions for many real world problems. 
% First, note that

% The main theoretical contribution of this paper is to give an affirmative answer to the  following question in positive 
% %ask the following two questions and answer them both in the positive:
% \begin{center}
%     \emph{Can we address the curse of dimensionality in Equation~\eqref{eq:ubfull} when $\mathcal F$ contains only $s$-sparse functions?}
% \end{center}

% More precisely, in Section~\ref{sec:mainthm} we 
% provide an algorithm with statistical rates that are exponential in \(1/s\) instead of \(1/d\), as present in Equation~\ref{eq:ubfull} (see Theorem~\ref{thm:mainthm}). While the results in the main text only consider the case where the data lives in the continous hypercube $[0,1]^d$, we also present results for general metric spaces in Appendix~\red{where}. 

% \red{change} Furthermore, we discuss in Section~\ref{sec:experiment} how our results motivate future work on fast greedy algorithms that  may lead to important practical  applications.  



%Theorem~\ref{cor:rates} we show 


 % We show that this is indeed possible by providing algorithms  
 







% \subsection{Notation}
% \label{subsec:notation}
% We refer to data sets of size $n$ with  $D \in T^n$. In the main text of this paper we usually assume that $T = [0,1]^d$ is the hyper cube equipped with the $\ell_{\infty}$-metric and let
%  $ T_k = \{ 1/2k, \cdots , (2k-1)/2k\}^d$ be the centers of a minimal $1/2k$-covering of $T$ of size $N =k^d$. 
% We denote with $\measure(T)$ the set of probability measures on $T$ and we let $\mathcal{M}(T)$ denote the set of signed measures on $T$. Moreover, $\mu_D$ is the empirical measure of a data set $D$ and 
%  $\mathrm{Lap}(\lambda)$ is the Laplace distribution with zero mean and variance~$2 \lambda^2$. 
%  We denote the matrix vector-$1$-norm with  $\|.\|_1$, and use the standard big-O-notation and the symbols $\lesssim_d, \gtrsim_d, \asymp_d$ to hide universal constants only depending on $d$. Finally, we denote with $\triangle^{d-1} \subset \mathbb R^d$ the probability simplex and for any function $f: T \to T'$ denote with $f_{\#} :\mathcal{M}(T) \to \mathcal{M}(T')$ the push-forward operator $f_{\#} \mu(A) = \mu(f^{-1} (A))$. 


 
%Finally, we use the well-established notation $C(d, s) = \binom{d}{s}$.
 

 % \red{STADNARD NOTATION COMES HERE}
% Put here all the notation... 
% where $W_1$ is the $1$-Wasserstein distance. 



% of the discrete measures where the minimum is taken over all permutations $\sigma: \{1, \cdots, n \} \to \{1, \cdots, n \}$. 
%  For any set of indices $S \in \{1, \cdots, d\}$, let $\mu_S \in \measure([0,1]^s)$ the marginal measure on the dimensions contained in $S$. 







% \begin{itemize}
%     \item What if the data is sparse?  Assume that the data lives on a $s$-dimensional subspace (see Definition bla) 
% \item In this case there exists a private algorithm which is adaptive to the "sparsity" of the measure
% \end{itemize}








% \paragraph{Open problem: efficient heuristic algorithms} 




% While the theory presented in the paper is very general, if we apply the algorithm to the $d$-dimensional hypercube $\mathcal D = [0,1]^d$ equipped with the infinity norm $\|.\|_\infty$, we get that 

% \begin{equation}
% \label{eq:ubfull}
%     \mathbb E W_1(\mu, \nu) \lesssim \sqrt{d} \left( \frac{\log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}.
% \end{equation}
% This bound is tight up to log factors, as we obtain a lower bound of order
% \begin{equation}
%     \mathbb E W_1(\mu, \nu) \gtrsim \sqrt{d} \left( \frac{1}{n \epsilon}\right)^{1/s}.
% \end{equation}





==> Workshop/Section2_algo.tex <==

\section{Certified DP data generation}
\label{sec:algo}


We present a private data release procedure that follows the general framework sketched in Algorithm~\ref{alg:mainalgo}. Unlike existing approaches, in addition to a DP measure $\mathcal A(D)$, Algorithm~\ref{alg:mainalgo} also returns  a  certificate $\ub_{\proxyutilitytemp}$ for the maximal utility loss \eqref{eq:utilityloss} over the class of sparse $1$-Lipschitz functions.

 

\begin{algorithm}[htbp!]
\caption{Privacy-Preserving Data Generation Framework}\label{alg:mainalgo}
\begin{algorithmic}[1]
\Require Data set $D$, privacy parameters $\epsilon$%,  noise distribution~$\noisedist$,  query operator $\mathbb{T}$\\
\State  $v \gets \mathbb{T} \mu_D$ \label{lin:projection}
\State construct the $\epsilon$-DP vector $\nudp := v +  \eta$ with $ \eta\sim \noisedist$ %some random vector 
\label{lin:make_dp}
%\State optimize  $\mudp \in \arg\underset{\mu \in \probset}{\min}~~\utilitylossT(\nudp,  \mathbb T \mu)$ 
\State optimize  $\mudp \in \underset{\mu \in \probset}{ \argmin}~~\ub_{\proxyutilitytemp}(\nudp,  \mathbb T \mu)$ 
\label{lin:optimize}
\State \Return DP measure $\mathcal A(D) \gets \mudp$ and certificate $\ub_{\proxyutilitytemp}(\mudp, \nudp)$  for $\utilityloss(\mu_D, \mudp)$
%for the utility loss $\utilityloss(\mudp, \mu_D)$ %loss~\eqref{eq:utilityloss} 
\end{algorithmic}
\end{algorithm}





 A common  data release framework consists of three standard steps. First, a linear query operator $\queryop: \probset \to \R^{m}$ projects the empirical data distribution of the data set $D$ in the domain $T$, onto a high-dimensional Euclidean space $\R^{m}$. Moreover, let $\image{\mathbb T}$ be the image of $\mathbb T$  and  $\Tinv:  \image{\mathbb T} \to \probset$ be any right-inverse, defined as satisfying  $\mathbb T \Tinv \mathbb T = \mathbb T$. The second step is the standard privatization procedure of adding noise from some distribution $\noisedist$ to the queries. In the last step, we project back from the query space $\R^m$ to the space of probability measures. 
 In Algorithm~\ref{alg:mainalgo}, this third step is done by minimizing the upper bound from a DP certificate $\ub_{\proxyutilitytemp}$ for the utility loss $\utilityloss$. Moreover, unlike existing algorithms, we release in Step 4 the DP-measure $\mu_{\text{DP}}$ together with a certificate for the maximum utility loss. 


We now introduce  the following general DP certificate for the maximum utility loss~\eqref{eq:utilityloss} 
that applies  to any probability measure $\mu \in \probset$. 
% To do so, we introduce the following general DP certificate for the maximum utility loss~\eqref{eq:utilityloss} 
%that applies  to any probability measure $\mu \in \probset$. 
For any DP-vector $\nudp := \queryop \mu_D + \eta$ 
as in Algorithm~\ref{alg:mainalgo},
we define
\begin{equation}
\label{eq:pluginub}
    \ub_{\proxyutilitytemp}(\mu, \nudp) := \underbrace{\sup_{\tilde \mu \in \probset} \utilityloss(\tilde \mu,\Tinv\mathbb T\tilde \mu)}_{\text{discretization error}}
   +\underbrace{ q_{1-\delta}\left(\proxyutilitytemp(0, \eta)\right)}_{\text{privatization error}}
   + ~\underbrace{\proxyutilitytemp(   \nudp,\mathbb T\mu) + \utilityloss(\Tinv \mathbb T\mu, \mu)}_{\text{projection error}}
\end{equation}
where $q_{1-\delta}(Z)$ denotes the $1-\delta$-quantile of the random variable $Z$ and $\proxyutilitytemp$ is a ''proxy" utility loss:

% such that for any vectors $v, v' \in \image{\mathbb T} \subseteq \mathbb R^m$,


\begin{definition}
\label{def:utilityloss} We say that $\proxyutilitytemp: \mathbb R^\Tdim \times \mathbb R^\Tdim \to \mathbb R$ is a proxy utility loss on $\mathbb R^\Tdim$ (\emph{dominating $\utilityloss$}) if for a right-inverse $\Tinv$ and for all $v, v' \in \image{\mathbb T} \subseteq \mathbb R^m$, 
$    \utilityloss(\Tinv v, \Tinv v') \leq \proxyutilitytemp(v, v').$
Moreover,  $\proxyutilitytemp$ is jointly translation invariant, that is $ \proxyutilitytemp(v, v') = \utilityloss(v + u, v' + u)$ for any $v, v', u \in \mathbb R^m$, and satisfies the triangle inequality. 
\end{definition}
% \begin{equation}
%    \proxyutility(u,v) = \utilityloss(\Tinv u, \Tinv v).
%    \label{eq:UT}
% \end{equation}
% Moreover, we say $\proxyutility$ is jointly translation invariant when $ \proxyutility(v, v') = \utilityloss(v + u, v' + u)$ for any $v, v', u \in \mathbb R^m$.
By the following lemma, $\ub_{\proxyutilitytemp}(\mu, \nudp)$ is indeed a high probability upper bound for the utility loss.
\begin{lemma}
\label{lm:upperbound}
For any proxy utility loss  $\proxyutilitytemp$ from Definition~\ref{def:utilityloss} and for $\nudp=\queryop \mu_D+\eta$ with $\eta \sim \noisedist$, we have that with probability $1- \delta$ over $\eta$ (for any $\delta>0$),  it holds that uniformly over all probability measures $\mu \in \probset$, we have $
\utilityloss(\mu_D, \mu) \leq\ub_{\proxyutilitytemp}(\mu, \nudp).$
\end{lemma}
\paragraph{Proof}
Using the triangle inequality and Definition~\eqref{def:utilityloss}, we can upper bound the utility loss for any $\mu \in \probset$ and $\mu_D$ by
\begin{align}
   \utilityloss(\mu_D, \mu) 
   &\leq \utilityloss(\mu_D,\Tinv \mathbb T\mu_D)+\utilityloss(\Tinv \mathbb T\mu_D, \Tinv \mathbb T\mu) + \utilityloss(\Tinv \mathbb T\mu, \mu)
   \nonumber \\
      &\leq \utilityloss(\mu_D,\Tinv \mathbb T\mu_D)+\proxyutilitytemp( \mathbb T\mu_D,  \mathbb T\mu) + \utilityloss(\Tinv \mathbb T\mu, \mu)
   \nonumber \\
   &\leq \utilityloss(\mu_D,\Tinv \mathbb T\mu_D)+\proxyutilitytemp( \mathbb T\mu_D,  \nudp )+\proxyutilitytemp(   \nudp,  \mathbb T\mu) + \utilityloss(\Tinv \mathbb T\mu, \mu)\nonumber\\
   &= \utilityloss(\mu_D,\Tinv \mathbb T\mu_D) + 
\proxyutilitytemp(0,   \eta ) + 
\proxyutilitytemp(    \nudp, \mathbb T\mu) + \utilityloss(\Tinv \mathbb T\mu, \mu)
\label{eq:general_ub123}
\end{align}
where in the last equality we used that $\nudp = \queryop \mu_D + \eta$ and the joint translation invariance of $\proxyutilitytemp$.


The first term can be described as the discretization error associated with $\Tinv \mathbb T$ and can be bounded by the supremum over all probability measures. 
Since we know the noise distribution $\noisedist$, the second term can be upper bounded with high probability by its $(1-\delta)$-quantile.
Finally, the third term only depends on $\mu$ and $\nudp$, which is DP by construction, and the fourth term only on $\mu$. 
As a result, we obtain the desired DP upper bound from Equation~\eqref{eq:pluginub}. 
\qed

\paragraph{Instantiating  Algorithm~\ref{alg:mainalgo} for sparse Lipschtiz functions}
We describe the specific instantiation of Algorithm~\ref{alg:mainalgo} in Appendix~\ref{sec:algo_instantioation}. Like previous works \cite{aim,mst}, we choose $\mathbb T$ to be the operator returning a vector representing all (discretized) marginal measures. The main difference to the mentioned papers lies in the construction of the proxy utility loss used in  Step~3 in Algorithm~\ref{alg:mainalgo}. This opens up the pathway for practically efficient extensions of our algorithm based on the extensions in  \cite{aim,mst} of the standard DP data generation framework. 











% Moreover, we mention that the certificates $\ub_{\utilitylossT}$ and $\ub_{\proxyutility}$ in Algorithm~\ref{alg:mainalgo} apply to any measure $\mu$, and therefore also to any approximate solution of the optimization problem in Step 3 in Algorithm~\ref{alg:mainalgo}. This opens up the path-way for future work on novel fast approximate algorithms with practically useful applications. 



==> Workshop/Section3_analysis.tex <==
% \section{Main result: Private data release for ``low-dimensional" data}

% The upper bound in Equation~\eqref{eq:ubfull} holds for any choice of the data set $D$ and is therefore a worst-case result. Our first main result of this paper demonstrates that
% these rates can be significantly improved when the data  lies on a low dimensional subspace. 
% As we show, this is  the case even when we do not have access to any oracle knowledge about the data set as the algorithm is capable of ``adapting'' to the data set. 
 
% For simplicity, here in the main text we only consider the setting where the underlying space is the $d$-dimensional hypercube equipped with the $\ell_{\infty}$-metric and refer the reader to Appendix~\red{where} for a general result. We now state our first main result:
% % As an outcome of Theorem~\ref{thm:mainthmmeasure} in Section~\ref{sec:mainmeasure}, we obtain Corollary~\ref{cor:ratesmeasure} state below. 
% % We refer the reader to Appendix~\ref{apx:mainmeasure} for the proof. 
% \begin{theorem}
% \label{cor:ratesmeasure}
% Let $c\geq 0$ be any constant and let $\mathcal F$ be the set of all $1$-Lipschtiz continuous functions on~$T = [0,1]^d$ with respect to the $\ell_{\infty}$-metric. 
% For any $n\epsilon \geq d+1$, there exists an $\epsilon$-DP algorithm $\mathcal A$ such that for any data set $D$,
% \begin{equation}
%     \label{eq:ratesmeasure}
%     \mathbb E ~\utilityloss (\mu_D, \algoD) \lesssim_{s}   \left( \frac{d^3 \log(\epsilon n)}{n \epsilon}\right)^{1/(s+1)} + \frac{d^2 \log(n\epsilon)^2}{n \epsilon^2},
% \end{equation}
% where $s\in \{0, \cdots, d\}$ is the smallest integer such that for all $k\geq 1$, $D$ is contained in at most $c k^s$ $\ell_{\infty}$-balls of radius   $1/2k$ with centers in $T_k$ (as defined in Section~\ref{subsec:notation}). 
% \end{theorem}
% The constant $s$ can be intuitively understood as the pseudo-dimension of the dataset $D$ and resembles the definition of the Minkowski dimension of a $s$-dimensional subspace of $T$. 
% Indeed, assuming that $D$ lives on a low dimensional sub-space, naturally we expect that only a few $\ell_\infty$-balls from the covering of $T$ with centers $T_k$ suffice to cover $D$. 







% The algorithm in Corollary~\ref{cor:ratesmeasure} is ``adaptive" in the sense that it adjusts to the characteristic $s$ of the data set without relying on any prior information or oracle knowledge of $s$. When the worst case scenario occurs and $s = d$, the rate in Equation~\eqref{eq:ratesmeasure} includes an additional term with an exponent of $+1$ compared to Equation~\eqref{eq:ubfull}. This raises the question of whether the cost of adaptivity can be reduced further, which remains an open problem for future research.

% \subsection{Description of the algorithm}

% We now describe the algorithm. 

% \paragraph{Step 1: construction of $\mathbb T$}

% \paragraph{Step 2: construction of $\nudp$}

% \paragraph{Step 3: choice of loss function $\utilitylossT$}



==> Workshop/Section4_example.tex <==





%  \subsubsection*{Acknowledgments}
% K.D.\ is supported by the ETH AI Center and the ETH Foundations of
% Data Science. A.S. is supported by the ETH AI Center. We would further
% like to thank Afonso Bandeira for insightful discussions.

 % We refer to Appendix~\ref{apx:experiments} for numerical simulations illustrating this upper bound.

 
 
 
 % in $\text{poly}(d^s k^s)$ run-time complexity for any $v \in \mathbb 
 % R^\Tdim$. 
 
 
 % In particular, let $\mu_{D'}$ be the empirical measure of any data set $D' \in T_k^m$ with $m$ some integer (where $T_k$ are the centers of the $1/2k$-covering of $T$) found via running a greedy algorithm minimizing 
 % $\utilitylossT(\nudp, \mathbb T \mu_{D'})$ in polynomial run time.
 %We present numerical simulations in Appendix~\ref{apx:experiments}. 

 
 
 
 

 
 
 
 
 
 % We therefore motivate future research on greedy algorithms which efficiently find solutions $D' \in T^m$ (with $m = O(\text{poly}(n))$ approximately minimizing $\utilitylossT(\nudp, \mathbb T \mu_{D'})$.

 
 
 % --- the computational ``hardness'' lies in finding a measure such that $\mathbb T \mu = v$ is an optimal solution. 
 
 
 
 

 
 
 
 % The only compuational ``hard'' part is to optimize 


% Implementing the instantiation of Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthmmeasure} is not trivial due to the difficulty in computing the loss function $\utilitylossT$. We therefore focus in this discussion on the instantiation of Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthm} which has the ``slow'' run-time complexity of order $\text{poly}(k^d,n)$ 
%  when $t=1/2k$  and $T=[0,1]^d$ is the hypercube equipped with the $\ell_{\infty}$-metric.



 
 


 

% The instantiation of Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthm} is not efficient in the sense that the  
% In this last section we discuss the efficient implementations which 
% for the Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthm} when being instantiated on the hypercube




% aspects of the our main results and motivate future work. 


% When again considering the case where $t=[0,1]^d$ is the hypercube and equipped with the $\ell_{\infty}$ metric, it is not difficult to see that the algorithms in Theorem~\ref{thm:march} and \ref{thm:mainthm} have a run-time complexity of $O(\text{poly}(k^d,n))$ where we discretize the hypercube into $k^d$ $\ell_{\infty}$ balls and thus $t=1/2k$. Furthermore, implementing the algorithm in Theorem~\ref{thm:mainthmmeasure} is non-trivial and its run time unclear. 






% \subsection{Open problems:}\red{Amartya:this should probably merge with conclusion}
% We motivate two open problems resulting from this paper for future work. 
% The first problem concerns tight bounds: We provide in Corollary~\ref{cr:lowerbound} in Appendix~\ref{apx:lowerbound} a lower bound for the worst case measure $\mu_D$ of order $ \mathbb E \utilityloss (\mu_D, \algoD) \gtrsim_s  \left( \frac{d\log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}$. This shows that our upper bound in Corollary~\ref{cor:rates} is tight in $n$ up to logarithmic factors but not in $d$. Closing this gap is a challenging task for future research as we believe that novel proof ideas are necessary. 

% Furthermore, as a second problem we motivate the development of  greedy algorithms for solving the optimization problem in Equation~\eqref{eq:heuristics} without using public data and polynomial run-time algorithms which provide approximate guarantees for an approximate version of the utility loss $\utilityloss$. 













% we can simply add and substract constants





% However, when $\mathcal F$ is the set of all $1$-Lipschitz continuous functions we have $\tilde  \utilitylossT(v, v') = \infty$ if $\|v\|_1 \neq \|v'\|$, making such a loss function infeasible. 


% First note that we can assume without loss of generality that $\mathcal F$





% We again first state the proof of Corollary~\ref{cor:ratesmeasure} and the present in Section~\ref{subsec:proofmeasure} the proof of the theorem. 
% \paragraph{Proof of Corollary~\ref{cor:ratesmeasure}}











% This result can be understood as an adaptivity statement for releasing private measures. 



% % Our result stands in analogy to adaptivity results for the prediction error in machine learning.













% We first present in Section~\ref{subsec:numerical} numerical simulations illustrating the upper bound in Theorem~\ref{thm:mainthm}, followed by a discuss of directions for practically efficient implementations in Section~\ref{sec:practical}
% \subsection{Numerical simulations}
% \label{subsec:numerical}

% The content in this section is:
% \begin{enumerate}
%     \item When instantiating the upper bound (we can even tighten the uppper bound) we obtain 
%     ....
%     \item we now compare this with the actul wasserstein distance of the loss
% \end{enumerate}



% \subsection{Practical aspects}
% \label{subsec:practical}


% Although Corollary~\ref{cor:rates} allows to overcome the course of dimensionality when choosing $s$ small, implementations of Algorithm~\ref{alg:mainalgo} have run-time complexity $\text{poly}(k^d)$ with $k = \frac{1}{2t}$. 




% \begin{enumerate}
%     \item When instantiating the upper bound (we can even tighten the uppper bound) we obtain 
%     ....
%     \item we now compare this with the actul wasserstein distance of the loss
% \end{enumerate}























   





% We now discuss the case where the dataset $T \subset \mathbb R^d$ is a compact subset of $\mathbb R^d$ and the goal is to construct an DP algorithm which achieves high utility on sparse Lipschitz continuous functions. 
% \red{Say something about the importance of this problem}


% In this section, we do bla bla


% For simplicity, for the following discussion we choose $T = [0,1]^d$ to be the $d$-dimensional hypercube and let $\mathcal F$ be the set of $s$-sparse Lispchitz continuous functions (i.e. $f$ only depends on $s$-dimensions),
% \begin{equation}
%     \mathcal F_s := \{f\vert~ f~1\text{-Lipschitz~w.r.t. }\|.\|_{\infty}\text{-norm~and~} f~\text{is}~s\text{-sparse}\}.
% \end{equation}
% To obtain an upper bound for the utility loss, we can apply Theorem~\ref{thm:mainthm} which yields the following corollary when using that $K ={d \choose s}$, 
% \begin{equation}
% N(T_{(i)}, \|.\|_{\infty},t) \leq (1/t)^s
% \end{equation}
%  and after optimizing over $t$:
% \begin{corollary}
% For any $n,d$ sufficiently large with $n\epsilon \geq d$ and constant $s$,  
% there exists an $\epsilon$-DP algorithm such that
% \begin{equation}
% \label{eq:ubfull}
%     \mathbb E U_{\mathcal F_s}(\mu_D, \algoD) \lesssim \sqrt{d} \left( \frac{\log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}.
% \end{equation}
% Furthermore, there exists an $(\epsilon,\delta)$-DP algorithm such that almost surely, 
% \begin{equation}
% \label{eq:ubfull}
%      U_{\mathcal F_s}(\mu_D, \algoD) \lesssim \sqrt{d} \left( \frac{\log(\epsilon n)^{2} \log(1 + \frac{e^\epsilon -1}{2 \delta})}{n \epsilon}\right)^{1/s}.
% \end{equation}
% \end{corollary}





% This bound is tight up to log factors, as we obtain a lower bound of order



% \begin{proposition}
% Lower bound
% \begin{equation}
%     \mathbb E W_1(\mu, v) \gtrsim \sqrt{d} \left( \frac{1}{n \epsilon}\right)^{1/s}.
% \end{equation}
% \end{proposition}


% \subsection{Efficient algorithms}





% \subsection{Numerical experiments}








% metrically private Algorithms. By  an algorithm $\mathcal A: \measure_0 \to \measure_1$ is $\epsilon$-DP if and only if $\mathcal A$ is $\epsilon n$-metrically private with respect to the normalized Hamming distance $\rho_1$. That is, for all measures $\mu_D, \mu_{D'} \in \measure_0$ and any subset of measures $V \subset \measure_1$ we have that
% \begin{align}
%     \frac{\mathbb P( \algoD \in V)}{\mathbb P( \mathcal A(\mu_{D'}) \in V)}\leq \exp\left(\epsilon n \rho_0(\mu_D, \mu_{D'})\right).
% \end{align}


==> macros/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\newcommand{\Tinv}[]{\mathbb{T}_R^{-1}}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.




==> sections/old_sections/Section1_intro.tex <==


\begin{abstract}
Differential privacy is the de facto standard for protecting privacy in a variety of applications. One of the key challenges is private data release, which is particularly relevant in scenarios where limited information about the desired statistics is available beforehand. Recent work has presented a differentially private data release algorithm that achieves optimal rates of order $n^{-1/d}$, with $n$ being the size of the dataset and $d$ being the dimension, for the worst-case error over all Lipschitz continuous statistics. This type of guarantee is desirable in many practical applications, as  for instance it ensures that clusters present in the data are preserved. However, due to the "slow" rates, it is often infeasible in practice unless the dimension of the data is small. We demonstrate that these rates can be significantly improved to $n^{-1/s}$ when only guarantees over s-sparse Lipschitz continuous functions are required, or to $n^{-1/(s+1)}$ when the data lies on an unknown s-dimensional subspace, disregarding logarithmic factors. We therefore obtain practically meaningful rates for moderate constants $s$ which motivates future work on computationally efficient approximate algorithms for this~problem.
\end{abstract}
% \begin{keywords}%
% Differential Privacy, Data Sanitization, Private Data Release\end{keywords}


\section{Introduction}
\let\thefootnote\relax\footnotetext{$^*$ Equal contribution; email address  konstantin.donhauser@ai.ethz.ch}
With increasing use of personal information in modern data analysis, 
guaranteeing the privacy of individual data points has become crucial.
Differential privacy
(DP)~\citep{dwork2006calibrating} 
has found its way into privacy protection 
%has grown to become the de-facto
%standard for privacy protection 
in both governmental \citep{Census} and commercial applications \citep{industry_eps}.
Intuitively, differential privacy guarantees that no single data point has a
significant impact on the output of the algorithm.  A probabilistic
algorithm $\mathcal{A}$ is said to be $\epsilon$-DP 
if it satisfies the conditions in
Definition~\ref{eq:defdp}. 

\begin{definition}
\label{eq:defdp}
    An algorithm $\gA$ is $\epsilon$-DP with $\epsilon>0$ if for any datasets $D, D'$ differing in a single entry and any measurable subset $S \subset \mathrm{im}(\mathcal A)$ of the image of $\mathcal A$, we have
    %\footnote{Commonly a slightly more general notion of DP is used where the algorithm $\mathcal A$ takes the dataset $D$ as input and therefore may also be sensitive to permutations of the dataset.}
\begin{equation*}
  \f{\P}{\f{\gA}{D}\in S} \leq \exp\brace{\epsilon} \f{\P}{\f{\gA}{D'}\in S}% + \delta
\end{equation*}
% where $\mu_D$ is the empirical measure of $D$.
\end{definition}
A long line of work focuses on preserving differential privacy while
extracting specific information from data,
%completing specific, a-priori known tasks on data, 
such as executing machine learning
algorithms~\citep{raskhodnikova2008can,chaudhuri2011differentially,feldman2014sample,bassily2014private}
or answering a number of pre-defined queries, see e.g.~\citet{dwork2004privacy,blum2005practical,hardt2010geometry,steinke2016between,ghazi21union,dagan2022bounded}.
%in a differentially private manner. 
Another line of work aims to preserve differential privacy for a-priori unknown queries from a large function class by releasing a synthetic data set \citep{blum2013learning,hardt2010multiplicative,mwem,liu2021iterative}. %that is differentially private with respect to a whole set of queries.
%However, in many situations, different users may like to use a dataset 
%request different statistics from the data and anticipating the needs of all potential users in advance can often be very challenging; this is for instance the case for census data~\citep{Census}. To address this shortcoming, a common solution is to release a differentially private, synthetic data set. 

This approach, also known as ``data sanitization"~\citep{dwork2009complexity}, provides guarantees over a class of queries, denoted as $\mathcal F$. Formally, we seek an algorithm $\mathcal A$ that takes  a data set $D$  as input and returns a probability measure $\mathcal A(D)$. This algorithm should have a low utility loss when applied to the predetermined class of functions or queries $\mathcal F$:
\begin{equation}
\label{eq:utilityloss}
    \utilityloss(\mu_D, \mathcal A(D) ) := \sup_{f\in \mathcal F} \left\vert \int f(x) d\mu_D - \int  f(z) d\algoD \right\vert 
\end{equation}

%\fy{sorry to write again, but still i would say if its whp or expectation and link to other peoples}

When designing such algorithms, we are faced with two key challenges:
(1) there is a natural trade-off between the statistical rates for the
utility loss and the complexity of the class of queries $\mathcal F$
and (2) algorithms with non-trivial guarantees for the utility loss
often run beyond polynomial time in the dimension of the data.
% algorithms with non-trivial guarantees for the utility loss are often NP-hard in the dimension of the data, unless the function class is simple. - too long, maybe split into two?}.
%\fy{unclear} For instance, \citet{dwork2009complexity,ullman2011pcps} give evidence for computational hardness for preserving second moments. T
This paper focuses on exploring the trade-offs in (1), but the results also motivate future research on developing novel efficient algorithms  for specific function classes~(2), as described in Section~\ref{sec:experiment}.

% \fy{not just the queries are restricted but also the domain (except wang, march). }
%\fy{focused on the linear or counting queries where the domain of the queries is discrete.}
Existing research on private data release has so far focused on
discrete domains such as counting, linear queries
or $k$-way marginals (see Appendix~\ref{sec:relatedwork} for an
overview).
%either focused on uniform bounds for general function classes~$\mathcal F$ \citep{blum2013learning}, discrete domains such as histograms \citep{nelson2019sok} or counting queries and $k$-way marginals (see Appendix~\ref{sec:relatedwork} for an overview).
% the rather
%  restrictive, but practically relevant cases where $\mathcal F$ 
%  is a
%  predefined finite set of query functions 
% \citep{blum2013fast,mwem,liu2021iterative} or 
In contrast, %Another direction has been recently taken by
~\citet{wang2016differentially,boedihardjo2022private} recently
studied continuous queries on continuous domains, e.g. the class of
all $1$-Lipschitz continuous functions.
Note that in this case, by the Kantorovich-Rubinstein
duality Theorem \citep{Villani2008OptimalTO}, the utility
loss~\eqref{eq:utilityloss} is equivalent to the $1$-Wassterstein
distance, also known as the \emph{earth mover's distance}. This
distance has also been widely used in machine learning, such as to design loss functions  \citep{frogner2015learning} or in combination with
optimal transport \citep{torres2021survey}, but also e.g., GAN's
\citep{Arjovsky17} and image retrieval \citep{rubner2000earth}.
Furthermore, a small Wasserstein distance is desired in many practical
applications as it guarantees that clusters present in the data remain
preserved (see the discussion in \citet{boedihardjo2022private}). 
% desirable 
% a practical viewpoint, a small earth mover's distance between the empirical measure $\mu_D$ and the private measure $\algoD$ is clearly desirable since Section~\citep{boedihardjo2022private})
% to the continuous domain as well as smooth functions.
%~\citet{boedihardjo2022private} pioneered a novel analysis which leads to  tight guarantees when $\mathcal F$ is the class of all
%$1$-Lipschitz continuous functions with respect to some metric. %\red{Maybe say why earth mover is practically relevant?}

When instantiated for the $d$-dimensional hypercube $[0,1]^d$ equipped with the
$\ell_{\infty}$-metric,  Corollary 9.2 in \citep{boedihardjo2022private} shows that there exists
an $\epsilon$-DP algorithm with expected utility loss at most 
\begin{equation}
\label{eq:ubfull}
    \mathbb E ~ \utilityloss(\mu_D, \algoD) \lesssim  \left( \frac{ \log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/d},
\end{equation}
where $n$ is the size of the data set $D$ and $\mu_D$ the corresponding empirical measure. In fact, without further
restrictions on the data set $D$, this rate is tight up to logarithmic
factors in $n$, and a concurrent work to this paper even shows that these logarithmic factors can indeed be removed \citep{Yiyun23}.
As a result, asking for such guarantees is practically
only feasible if the dimension $d$ of the dataset is small. In this
work, we ask the following two questions and answer them both in the positive:

\begin{center}
    \emph{Can we address the curse of dimensionality in Equation~\eqref{eq:ubfull} when (1) $\mathcal F$ contains only $s$-sparse functions or (2) the data $D$ lies on a low-dimensional subspace.}
\end{center}

 We show that this is indeed possible by providing algorithms with statistical rates that are exponential in \(1/s\) instead of \(1/d\), as present in Equation~\ref{eq:ubfull}. Furthermore, we discuss in Section~\ref{sec:experiment} how our results motivate future work on fast greedy algorithms that  may lead to important practical  applications.  
 %In agreement with existing computational hardness results \citep{dwork2009complexity,ullman2011pcps}, the presented algorithms are not computationally efficient. However, as we discuss in Section~\ref{sec:experiment}, our results open up the pathway for the development of fast greedy algorithms that  might lead to important practical  uses cases. 




 % our algorithmswhich motivates future research on developing efficient heuristics to increase its practical utility.
% \fy{implies new research for comput. efficient bla (also to already mention that its not efficient...?}





% and thus choosing $\mathcal F$ 

% This paper primarily





% overcome the limitations approach is often 
% an approach, however, is 
% the use-cases of the data  strongly among the users,
% study the  when the use of the data is not known in advance or may vary strongly among the users, an alternative is to release a synthetic datasets, 





% In many cases however, such as it is for instance the case for census data \citep{census}, different users may ask for 
% different statistics from the data which are also difficult to anticipate in advance. 

% %the data. 

% which different users would like from the data may vary strongly and is

% of data may strongly vary among the different users. 



% In many cases however, various users 



% To overcome the limitations approach is often 
% an approach, however, is 
% the use-cases of the data  strongly among the users,
% study the  when the use of the data is not known in advance or may vary strongly among the users, an alternative is to release a synthetic datasets, often called ``sanitisation"~\citep{blum2013learning,dwork2009complexity}. 
% The most commonly
% researched setting is when the performed tasks on the data are known in advance, such as answering of a finite set of pre-defined queries \red{cite} or running a machine learning algorithm 
% the algorithm or the list of queries are
% known in advance  An extensive line of research studies the problem where the use of the data is known in advance, 
% Assuming that the use-cases of the data are known in advance, such running a machine learning algorithm or answering a finite set of predefined queries, there exists a long line of
% work~\citep{raskhodnikova2008can,feldman2014sample,bassily2014private,chaudhuri2011differentially} which shows
% how to construct differentially private learning algorithms. However,
% this requires knowing the learning task in advance and also designing
% specific algorithms for separate problems.
% Another line of work that is more relevant to ours is that of
%``sanitisation"~\citep{blum2013learning,dwork2009complexity} where the
% private data is released to the public in the form of a synthetic
% dataset.
%The advantage of such algorithms is that we do not need to know the
% precise use of the In contrast to the previous approach, once the
% sanitised dataset is released, any function~(also referred to as
% query) can be applied on the dataset without violating its privacy;
% the caveat being that only certain functions are guaranteed to
% output a result close what it would have output on the original
% private dataset. We refer to Section~\ref{subsec:relatedwork} for a
% summary of the related work on this topic.










% a set of linear functions \red{cite} or linear thresholding functions \cred{cite} or a set of marginal queries $f(z) = \delta($











% \textbf{First paragraph:} (Privacy is important)
% \begin{enumerate}
%     \item  Privacy is a  crucial problem
% \item Albeit there exists many different definitions for a private algorithm [cite], most common definition is DP
% \item State definition
% mention why it is so popular, also used in industry by big tech and other place. 
% \end{enumerate}




% \textbf{Third paragraph:}(alternative, private data release)
% \begin{enumerate}
%     \item An alternative consists of releasing a synthetic dataset which is private. 
% \item So far, existing works focussed on 
% \item Many heuristic algorithms without guarantees
% \item Histogram clustering algorithms
% \item Respect only $s$-marginals
% \end{enumerate}




% \textbf{Fourt paragraph:} For a function class $\mathcal F$, we are interested in algorithms which give guarantees for 

% Following the ideas



% \red{\paragraph{Related work \citep{boedihardjo2022private}: $\mathcal F = \mathcal F_{\text{Lip}}$}}
% is the set of all Lipschtiz continuous functions
% Let $(T, \rho)$ be a metric space. 

% Note that when $s=d$, the utility loss is exactly the 1-Wasserstein distance of the corresponding empirical measures $\mu$ and $\nu$, i.e., 





% While the theory presented in the paper is very general, if we apply the algorithm to the $d$-dimensional hypercube $\mathcal D = [0,1]^d$ equipped with the infinity norm $\|.\|_\infty$, we get that 




% In order to relate measures to a dataset, we will be considering empirical measures. Formally, for some dataset $D$ we denote its empirical distribution as $\mu_D = \sum_{x \in D} \frac{1}{\vert D \vert} \delta_x$. 

\subsection{Main result: Private data release for sparse function classes}
\label{subsec:mainresultsparse}
To the best of our knowledge, we are the first to explicitly study the
case where $\mathcal F$ is the set of $s$-sparse $1$-Lipschitz
continuous functions (i.e.  functions that only depend on
$s$-dimensions of the input).  In particular,
Corollary~\ref{cor:rates} of our main Theorem~\ref{thm:mainthm} shows
how
%As we show below in Corollary~\ref{cor:rates}, which is an outcome of our main result Theorem~\ref{thm:mainthm} in Section~\ref{sec:mainthm}, 
restricting $\mathcal F$ to sparse functions significantly improves the rates for the utility loss~\eqref{eq:utilityloss}, and thereby allows us to effectively overcome the curse of dimensionality in Equation~\eqref{eq:ubfull}. 
The improvement of the rate exponent from $1/d$ in Equation~\eqref{eq:ubfull} to $1/s$ is, in fact, tight by Corollary 9.4 in \citep{boedihardjo2022private}. 
Furthermore, the dependency on the dimension $d$ is now only linear; and we pose it as an open problem to improve this dependency to $d^{1/s}$, which would match the lower bound of order $ \left( \floor{\frac{d}{s}}\frac{1}{n \epsilon}\right)^{1/s}$ 
obtained from a straightforward modification of Corollary 9.4 in \citep{boedihardjo2022private}.%, 

\begin{corollary}(of Theorem~\ref{thm:mainthm})
\label{cor:rates}
Let $\mathcal F$ be the set of $s$-sparse $1$-Lipschitz continuous functions on $[0,1]^d$ with respect to the $\ell_{\infty}$-metric. Then, for any $n\epsilon \geq d$ and any $s\leq d$, there exists an $\epsilon$-DP algorithm such that
\begin{equation}
\label{eq:ratessparse}
    \mathbb E ~\utilityloss (\mu_D, \algoD) \lesssim_s  ~d \left( \frac{ \log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}.
\end{equation}
%Equation~\eqref{eq:ratessparse} holds. 
\end{corollary}
We now argue for the relevance of 
%hat a small utility loss over the set of all 
$s$-sparse, $1$-Lipschitz continuous functions in practice. %results in practically meaningful guarantees for a wide range of applications. 
First, note that one of the most common uses of many data sets, such
as census data \citep{Census}, is to ask for the relationship among
different (few) features, e.g., the relationship between gender,
income, and job category. Such queries are, by nature, sparse
functions and can often be approximated using sparse,
Lipschitz-continuous functions. Furthermore, any (scaled) $s$-way
marginal $f(x) = \frac{1}{\vert S\vert} \prod_{i \in S} x_{i}$ with
$\vert S \vert \leq s$ is contained in $\mathcal F$, which is an
important problem that has been extensively studied in the privacy
literature (see Section~\ref{sec:relatedwork}).  Finally, we remark
that clusters on the projected subspaces are also preserved, since by the
Kantorovich-Rubinstein duality theorem \citep{Villani2008OptimalTO},
the utility loss is equal to the maximum $1$-Wasserstein distance over
all sparse marginals:
% We now argue that a small utility loss over the set of all $s$-sparse $1$-Lipschitz continuous functions still results in practically meaningful guarantees for a wide range of applications. First, note one of the most common use of many data sets such as census data \citep{Census} is to ask for the relation among different (few) features, such as how does the gender, income and job category relate etc., that are by nature sparse functions and can be approximated using (sparse) Lipschitz-continuous functions. Furthermore, any (scaled) $s$-way marginal $f(x) = \frac{1}{\vert S\vert }\prod_{i \in S} x_{i}$  with $\vert S \vert \leq s$ is contained in $\mathcal F$ --- which is itself an important extensively studied problem  in the privacy literature (see Section~\ref{sec:relatedwork}).  
% Finally, 
% we remark that also sparse clusters are preserved (see the discussion in \citet{boedihardjo2022private}), since by the Kantorovich-Rubinstein
%  duality Theorem \citep{Villani2008OptimalTO}, the utility loss is equal to the maximum $1$-Wasserstein distance over all sparse marginals: 
 %if $\mathcal F$
% is the set of $s$-sparse $1$-Lispchtiz continuous functions, we have
\begin{equation}
\label{eq:wassersteinsparse}
    \utilityloss(\mu_D, \algoD ) =  \sup_{S \subset \{1, \cdots, d\}; \vert S \vert =s} W_1 \left(\mu_{D}^{S}, \algoD^S\right),
\end{equation}
where  $W_1$ is the $1$-Wasserstein distance, and $\mu_{D}^{S}$ the marginal measure of $\mu_D$ on
the $s$-dimensional subspace defined by the coordinates in $S$. 






% While Corollary~\ref{cor:rates} shows that reducing $\mathcal F$ to only consider sparse functions yields a significant improvement in the rates for the utility loss~\eqref{eq:utilityloss}, 



% Releasing a data set with guarantees for any sparse Lipschitz
% statistics is significant in a range of practical applications, and especially 
% for data sets with moderate to high dimensions where the rates in Equation~\eqref{eq:ubfull} are too slow from a practical perspective. For instance, sparse counting queries are widely used for census data \citep{Census} and can approximated using Lipschitz-continuous soft-threshold functions. 



% include soft-thresholding functions in 
% For instance, 
% high-dimensional datasets like census and genomic data, useful queries
% often tend to depend on a few variables. 
%Our results shows how to
%release the census or genomic data in a differentially private way
%while guaranteeing small error in these queries.
% Furthermore, in the learning
% theoretic setting, our results also guarantee that sparse clusters present in the original non-private dataset are preserved in the
% generated private dataset. Indeed, by the Kantorovich-Rubinstein
% duality Theorem \citep{Villani2008OptimalTO}, if $\mathcal F$
% is the set of $s$-sparse $1$-Lispchtiz continuous functions, we have
% \begin{equation}
% \label{eq:wassersteinsparse}
%     \utilityloss(\mu_D, \algoD ) =  \sup_{S \subset \{1, \cdots, d\}; \vert S \vert =s} W_1 \left(\mu_{D}^{S}, \algoD^S\right),
% \end{equation}
% where  $W_1$ is the $1$-Wasserstein distance, and $\mu_{D}^{S}$ the marginal measure of $\mu_D$ on
% the $s$-dimensional subspace defined by the coordinates in $S$. 



% Our contribution is to show that we can effectively address the
% curse of dimensionality in the bound on the utility loss in
% Equation~\eqref{eq:ubfull} when choosing $s \ll d$.
% As a direct outcome of our main result Theorem~\ref{thm:mainthm} in Section~\ref{sec:mainthm}, we present Corollary~\ref{cor:rates} which shows that we can achieve significantly faster rates when restricting $\mathcal F$ to only contain sparse functions; thereby we effectively address the curse of dimensionality in Equation~\eqref{eq:ubfull}:
% by restricting the set of all $1$-Lipschitz
% continuous functions to the set of $s$-sparse  \(1\)-Lipschitz
% functions. Consider the underlying space to be the $d$-dimensional
% hypercube as in Equation~\eqref{eq:ubfull}. As a direct outcome of our main result, we present Corollary~\ref{cor:rates} that achieves significantly faster rates when restricting $\mathcal F$ to only contain sparse functions: 
% \begin{corollary}(of Theorem~\ref{thm:mainthm})
% \label{cor:rates}
% Let $\mathcal F$ be the set of $s$-sparse $1$-Lipschitz continuous functions on $[0,1]^d$ with respect to the $\ell_{\infty}$-metric. Then, for any $s\leq d$ there exists an $\epsilon$-DP algorithm such that
% \begin{equation}
% \label{eq:ratessparse}
%     \mathbb E ~\utilityloss (\mu_D, \algoD) \lesssim_s  ~d \left( \frac{ \log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}.
% \end{equation}
% %Equation~\eqref{eq:ratessparse} holds. 
% \end{corollary}
% Corollary~\ref{cor:rates} improves the exponent in the rates from $1/d$ in Equation~\eqref{eq:ubfull} to $1/s$, which is in fact tight  as a direct consequence of Corollary 9.4 in \citep{boedihardjo2022private}. 
% Furthermore, the dependency on the dimension $d$ is now linear, and we pose it as an open problem to improve this dependency to $d^{1/s}$, which would match the lower bound of order $ \left( \floor{d/s}\frac{1}{n \epsilon}\right)^{1/s}$
% which we obtain from a straight forward modification of Corollary 9.4 in \citep{boedihardjo2022private}.%, which we believe is optimal.% \red{We need to metion the h.p. guarantee}

% Furthermore, in Appendix~\ref{apx:experiments} we
% provide numerical simulations illustrating our upper bounds. However,
% our presented algorithm is not computationally efficient, which is
% expected due to existing computational hardness
% results~\citep{ullman2011pcps}. 

% Finally,  isolate in Section~\ref{sec:experiment}
% the computationally inefficient part of our algorithm~(Step 3 of
% Algorithm~\ref{alg:mainalgo}) in a way that many off-the-shelf
% optimisation algorithms and heuristics can be applied non-privately.
% As the optimisation methods are applied non-privately, the empirical
% loss of these methods is visible to the analyst and we show how to use
% this to provide a guarantee on the utility loss.

%\red{konstantin have a
%look here.}

% In Section~\ref{cr:lowerbound}, we show that the above bound is tight in the
% size of the dataset~(but not in dimension), up to logarithmic factors
% and in Section~\ref{sec:algo}, we present an algorithm to achieve this
% statistical rate. 




% In this setting, as a consequence of our abstract main result, Theorem~\ref{thm:mainthm} in
% Section~\ref{sec:mainthm}, we obtain
% the following upper bound for utility loss~\eqref{eq:utilityloss}:

%\fy{this looks a little strange - either put cor. informal or the full one (probz informal)}
% \red{WIP WIP}
% As our algorithm is computationally inefficient, we isolate
% the computationally inefficient part of our algorithm~(Step 3 of
% Algorithm~\ref{alg:mainalgo}) in a way that many off-the-shelf
% optimisation algorithms and heuristics can be applied non-privately. In Section~\ref{sec:experiment} we
% provide numerical simulations of our algorithm  ...\red{Not there yet}. 




\subsection{Main result: ``Low-dimensional" data}
%\label{sec:relatedwork}
% \red{I do not know any solid use cases though....}
%\red{Maybe we can call this Main Result 2 and the previous Main Result 1 ?}
The upper bound in Equation~\eqref{eq:ubfull} holds for any choice of the data set $D$ and is therefore a worst-case result. Our second main result of this paper demonstrates that
these rates can be significantly improved when the data  lies on a low dimensional subspace. 
As we show, this is  the case even when we do not have access to any oracle knowledge about the data set as the algorithm is capable of ``adapting'' to the data set. 
%(see Section~\ref{sec:mainmeasure} for a
%formal definition).

Consider the same setting as in Equation~\eqref{eq:ubfull}, where the underlying space is the $d$-dimensional hypercube $T =  [0,1]^d$ equipped with the $\ell_{\infty}$-metric. 
Let
$ T_k = \{ 1/2k, \cdots , (2k-1)/2k\}^d$
 be the centers of a minimal $1/2k$-covering of $T$ of size $N =k^d$. 
 % For any data set $D$ we define the pseudo-dimension of the data:
% \begin{definition}(pseudo-dimension of the data)
% For any constant $c$ and any data set $D$ let $s_c(D) \in \{0,\cdots, d\}$  be the smallest integer such that for all $k\geq 1$, $D$ is contained in at most $c k^s$ $\ell_{\infty}$-balls of radius   $1/2k$ with centers in $T_k$.
% \end{definition}
As an outcome of Theorem~\ref{thm:mainthmmeasure} in Section~\ref{sec:mainmeasure}, we obtain Corollary~\ref{cor:ratesmeasure} state below. 
% is  an outcome of our second main result 
% and shows that when the data set lies on a low-dimensional subspace (as made precise in the corollary), we can achieving significantly faster rates compared to the ones for the worst case data set in Equation~\eqref{eq:ubfull}. 
We refer the reader to Appendix~\ref{apx:mainmeasure} for the proof. 
\begin{corollary}(of Theorem~\ref{thm:mainthmmeasure})
\label{cor:ratesmeasure}
Let $c\geq 0$ be any constant and let $\mathcal F$ be the set of all $1$-Lipschtiz continuous functions on $[0,1]^d$ with respect to the $\ell_{\infty}$-metric. 
For any $n\epsilon \geq d+1$, there exists an $\epsilon$-DP algorithm $\mathcal A$ such that for any data set $D$,
\begin{equation}
    \label{eq:ratesmeasure}
    \mathbb E ~\utilityloss (\mu_D, \algoD) \lesssim_{s}   \left( \frac{d^3 \log(\epsilon n)}{n \epsilon}\right)^{1/(s+1)} + \frac{d^2 \log(n\epsilon)^2}{n \epsilon^2},
\end{equation}
%Equation~\eqref{eq:ratesmeasure} holds
where $s\in \{0, \cdots, d\}$ is the smallest integer such that for all $k\geq 1$, $D$ is contained in at most $c k^s$ $\ell_{\infty}$-balls of radius   $1/2k$ with centers in $T_k$.
% Furthermore, there exists an $(\epsilon,\delta)$-DP algorithm $\mathcal A$ such that almost surely, 
% \begin{equation}
% \label{eq:ubfull}
%      \utilityloss(\mu_D, \algoD) \lesssim_{s_c(D)} \left( \frac{d\log(\epsilon n) \log(1 + \frac{e^\epsilon -1}{2 \delta})}{n \epsilon}\right)^{1/(s_c(D)+1)}.
% \end{equation}
\end{corollary}
%The proof of the corollary follows from exactly same argument as the proof of Corollary~\ref{cor:rates} when using Theorem~\ref{thm:mainthmmeasure} below.
Note that the definition of $s$ in Corollary~\ref{cor:ratesmeasure} resembles the definition of the Minkowski dimension when the data set $D \subset T_s$ lives on a subspace $T_s$ of Minkowski dimension $s$. The algorithm in Corollary~\ref{cor:ratesmeasure} is ``adaptive" in the sense that it adjusts to the characteristic $s$ of the data set without relying on any prior information or oracle knowledge of $s$. When the worst case scenario occurs and $s = d$, the rate in Equation~\eqref{eq:ratesmeasure} includes an additional term with an exponent of $+1$ compared to Equation~\eqref{eq:ubfull}. This raises the question of whether the cost of adaptivity can be reduced further, which remains an open problem for future research.

% see that an additional $+1$ term appears in the exponent,


% When again considering the underlying space to be the $d$-dimensional
% hypercube as in Equation~\eqref{eq:ubfull},  as a consequence of our abstract main result, Theorem~\ref{thm:mainthmmeasure} in
% Section~\ref{sec:mainmeasure}, we obtain
% the following upper bound for utility loss~\eqref{eq:utilityloss}:
% we obtain
% the following corollary of our abstract main result in
% Section~\ref{sec:mainmeasure}:
% The previous result did not make any assumptions on the data
% distribution but restricted the class of functions to the set of
% sparse lipschitz queries.
% Our second result provides guarantees for a
% restricted set of data distributions but for all \(1\)-lipschitz
% queries. 

% Unlike~\citet{boedihardjo2021privacy}, who suffered the an
% exponential dependence on dimension for this class of queries, we show
% that restricting the data allows us to get rid of the curse of the
% dimensionality.


% In particular, we consider the case when the data lies on a
% \(s\)-dimensional subspace~(see Section~\ref{sec:mainmeasure} for a
% formal definition). In this setting, we propose an algorithm that
% ``adapts'' to the sparsity of the data i.e. gives a statistical rate
% which depends on the sparsity of the data. In particular, we provide
% the following upper bound on the utility loss


% where the utility loss is over the class of all $1$-Lipschitz continuous functions and $s\leq d$ is the dimension of the subspace the data set lives in. 


\subsection{Notation}
We use the standard big-Oh notation and the symbols $\lesssim_d, \gtrsim_d, \asymp_d$ to hide universal constants only depending on sub-script $d$. We use the notation $D \in T^n$ for data sets of size $n$ on a measurable space $(T, \mathcal B)$
with $\sigma$-algebra $\mathcal B$.  
Furthermore, we denote with $\measure(T)$ the set of probability measures on $T$ and let $\mu_D$ be the empirical measure of a data set $D$. 
For any two data sets $D,D'\in T^n$, we let $H(D, D')  = \vert  \{i \in \{1, \cdots, n \} \vert x_i \neq x'_{i}\} \vert$ be the Hamming distance and let $N(T, \rho, t)$ be the $t$-covering number of the metric space~$(T, \rho)$. 
 We let $\mathrm{Lap}(\lambda)$ be the Laplace distribution with zero mean and variance~$2 \lambda^2$.



% \red{STADNARD NOTATION COMES HERE}
% Put here all the notation... 
% where $W_1$ is the $1$-Wasserstein distance. 



% of the discrete measures where the minimum is taken over all permutations $\sigma: \{1, \cdots, n \} \to \{1, \cdots, n \}$. 
%  For any set of indices $S \in \{1, \cdots, d\}$, let $\mu_S \in \measure([0,1]^s)$ the marginal measure on the dimensions contained in $S$. 







% \begin{itemize}
%     \item What if the data is sparse?  Assume that the data lives on a $s$-dimensional subspace (see Definition bla) 
% \item In this case there exists a private algorithm which is adaptive to the "sparsity" of the measure
% \end{itemize}








% \paragraph{Open problem: efficient heuristic algorithms} 




% While the theory presented in the paper is very general, if we apply the algorithm to the $d$-dimensional hypercube $\mathcal D = [0,1]^d$ equipped with the infinity norm $\|.\|_\infty$, we get that 

% \begin{equation}
% \label{eq:ubfull}
%     \mathbb E W_1(\mu, \nu) \lesssim \sqrt{d} \left( \frac{\log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}.
% \end{equation}
% This bound is tight up to log factors, as we obtain a lower bound of order
% \begin{equation}
%     \mathbb E W_1(\mu, \nu) \gtrsim \sqrt{d} \left( \frac{1}{n \epsilon}\right)^{1/s}.
% \end{equation}





\section{Related work}
\label{sec:relatedwork}
% \textbf{Second paragraph:} (Existing Algorithms focus on queries or specific algorithms)
% \begin{enumerate}
%     \item A large body of work studies the problem of answering multiple queries privately, as well as privaticing existing specific algorithms such as SGD training.  
%     \item Most of these works have three steps: i) Measure
% \item Major disadvantage: need to know in advance what information about the data is required.
% \item Followup queries come with a sacrifice in privacy guarantees. 

% \end{enumerate}
Releasing datasets privately while minimizing the utility loss for a specific function class is a major challenge in differential privacy. Most studies have focused on preserving utility for counting queries (referred to as statistical queries in~\citet{kearns1998efficient}). The field started with~\cite{blum2013learning}, who applied the Exponential Mechanism algorithm of~\cite{mcsherry2007mechanism} to release a private dataset while ensuring that the loss of utility for any a priori known set of counting queries grows at most logarithmically with the set size. Subsequent works by~\citet{dwork2009complexity,roth2010median,hardt2010multiplicative,mwem} 
improved both the statistical and computational complexity and studied fundamental statistical-computational tradeoffs and gaps ~\citep{dwork2009complexity,ullman2011pcps}. In our paper, we focus on improving the statistical
and leave the development of an computationally efficient algorithm to future work.
%, but their algorithms were still exponential in the worst case; which indeed seems  to be unavoidable~\citep{dwork2009complexity,ullman2011pcps}. 

% \fy{i don't think we have to focus on comp. vs. ineff. - we are not giving a tutorial here. at the same time i would probably mention more of this work in intro and move to appendix, or shorten it and leave it here.}
%Previous work has considered 
In order to reduce sample complexity, several works have considered sparsity assumptions in various ways. 
For example, \citet{blum2013fast} propose an efficient algorithm for queries that take on a non-zero value only on a small subset of an unstructured discrete domain. More related to us, a special class of linear statistical or counting queries are k-way marginals~\citep{thaler2012faster,dwork2015efficient,liu2021iterative}. A k-way marginal query involves fixing the values of \(k\) indices and determining the proportion of data that matches those values.
Further, a range of works~\citep{Barak07,gupta2011privately,cheraghchi2012submodular} also study the query class of k-way conjunctions and provide fast algorithms when \(k\) is small. 
%Despite the hardness results in the worst case, some recent works have proposed using existing NP-hard optimization solvers, such as integer programming~\citep{gaboardi14,vietri2020new} and gradient-based methods~\citep{aydore2021differentially}, as subroutines in the private data release algorithm. This idea also applies to algorithms using a variation of the~\emph{Projection Mechanism} first developed in~\citep{nikolov2013geometry} and later improved in~\citet{dwork2015efficient,blasiok2019towards}. More generally, this line of work is referred to as~\emph{oracle efficient} algorithms and the optimality guarantee depends on the optimality of the oracle that solves the hard subroutine.
% The above works focus on optimality with respect to certain counting queries. Counting queries evaluate the proportion of the data that has a positive response to a specific query. 
%% Please fix how they're related...
Further common problems in the privacy literature related to this paper include histogram release 
\citep{hay2009boosting,xiao2010differential,acs2012differentially,qardaji2013understanding,xu2013differentially,zhang2016privtree,meng2017different,nelson2019sok,abowd2019census} and private clustering \citep{su2016differentially,balcan2017differentially,Stemmer20,ghazi2020differentially}.
  % A histogram, corresponding to a domain and a dataset, is simply the frequency of each domain element in that dataset and can provide useful summaries of the dataset. There has been a sizeable amount of work in the literature~\citep{privelet,nelson2019sok,acs2012differentially,hay2009boosting,qardaji2013understanding,meng2017different,xu2013differentially,zhang2016privtree,abowd2019census} towards releasing histograms privately.
 % While these are powerful queries, they do not guarantee that the released private data behaves in the same way as the original data under more general functions.~\citet{wang2016differentially,boedihardjo2022private} took an important step towards this issue by providing guarantee for the class of all 1-Lipschitz functions. However, their statistical complexity is ~(necessarily) very poor and depends exponentially on the dimension (see Equation~\eqref{eq:ubfull}). Inspired by~\citet{boedihardjo2022private}, we consider this more powerful setting of Lipschitz queries but avoid the exponential dependence of dimension by looking at sparse Lipschitz queries.

% \paragraph{Use of public data} Another line of work leverages public data for private data release.~\citet{bassily2020private} uses the public data, in a similar way as~\citet{alon2019limits}, to reduce the query set and then uses the algorithm of~\citet{hardt2010multiplicative} on this reduced query set. However, their algorithm is not necessarily computationally efficient. On the other hand~\citet{liu2021leveraging} leverages the public data to identify a smaller subset of the data domain and then run the algorithm of~\citet{mwem} on this. While this improves both the statistical and computational complexity of the algorithms, their setting is related to the weaker setting of counting queries. In addition, we use a similar strategy to show the practical utility of our algorithm in~\red{refer to app}.

% \paragraph{Deep learning techniques} Some recent works have also used modern deep learning techniques to generate private synthetic data.~\citet{beaulieu2019privacy,jordon2019pate,torkzadehmahani2019dp,neunhoeffer2020private} use a type of Generative Adversarial Network~(GAN), trained using Differentially Private SGD on private data to produce private synthetic data. On the other hand,~\citet{takagi2021p3gm} uses another kind of deep generative model known as Variational Auto Encoder~(VAE). However, neither do these methods come with any theoretical guarantees on their utility loss nor do they perform well in practice compared to the other approaches mentioned above.



% Using this definition we will we interested in understating the quantity $\mean{W_1(\mu_D, \mathcal{A}(D)}){}$ for a synthetic data generation algorithm $\mathcal{A}$ whose output is discrete measure over the data space. As any discrete measure can be approximated arbitrarily well, it suffices to study this setting.





% \paragraph{Background: March's paper \citep{boedihardjo2022private}}
% Previous work \citep{boedihardjo2022private} considers the case where $s=d$. The algorithm then consists of the following steps:


% \begin{theorem}
% For any $\epsilon,\delta$ there exists an $\epsilon, \delta$-DP algorithm which 
% \end{theorem}
% \begin{enumerate}
%     \item Discretize the data using a $\delta$-covering of the space. The data can then be represented as a discrete measure $\mu_D$ (which we can represent as an vector $\in \mathbb R^{N}$ with $N$ the size of the covering). For the infinity norm on the hypercube, we have $N= k^d$ with
%     $k = \ceil{1/\delta}$. 
%  \item We can then construct a new private (signed) measure $\nu_D = \mu_D + \Phi L$
%         where $\Phi$ is the Haarbasis and $L$ an i.i.d. random vector with Laplacians. The choice of the Haarbasis is crucial to obtain a small average error $\mathbb E W_1(\nu, \mu)$. 
%     \item In a last step, we convert $\mu_D$ into a probability measure and approximate it using $m$-samples $\{z_i\}_{i=1}^m$ (with $m\gg n$) (and hence obtain the desired measure $\nu$). 
% \end{enumerate}



==> sections/old_sections/Section2_algo.tex <==

\section{Abstract Privacy Preserving Data Generation}
\label{sec:algo}
In this section, we describe a standard framework for data generation
algorithms $\mathcal A$ which take a data set $D \in T^n$ of size $n$
as input, and 
% $\mu \in \probset$ \fy{also sounds a little weird empirical measure (i would say empirical measure on $n$ data points that are in domain $T$ - i'd say abstractly speaking, algorithm takes a measure and then say that effectively its the empirical distribution on $n$ datapoints. $n$ also appears out of nowhere later - also for some reason i think it's good to say that $T$ is gonna be instantiated on $d$-dim hypercube. } on a measurable space $T$ as input 
 output an $\epsilon$-DP  measure $\algoD\in \probset$. Described in
 Algorithm~\ref{alg:mainalgo}, this framework consists of three steps.
 The first step (1) projects the empirical measure $\mu_D$  to a
 finite-dimensional vector $v$. Step (2) generates a DP version
 $\nudp$ of this vector and finally, step (3) obtains a DP measure
 $\mathcal A(D)$ by minimizing a loss function between the vector
 $\nudp$ and the projection of $\mathcal A(D)$.  Since, in step (3),
 the information about the data $D$ is only used via the private
 vector $\nudp$, the outcome of the algorithm is then trivially DP.  
We refer to Appendix~\ref{apx:algoexample} for an example demonstrating how this framework applies to general function classes $\mathcal F$. %Algorithms following this pattern have been widely used in the literature (see e.g., \red{cite}) \fy{but for xxx - difference}.  
We now introduce each step of Algorithm~\ref{alg:mainalgo} more formally. 


% based on the (truncated) Laplace mechanism which
% The Laplace mechanism is a widely used tool to construct synthetic data generation \red{where} algorithms  in the literature \red{cite a bunch of them}. 


 % Algorithm~\ref{alg:mainalgo} consists of three steps, where the first two steps follow the standard
 % patterns (see e.g., \red{where}) while the third step allows for more generality over existing approaches.
\paragraph{Projection \textit{(1)} :}~the first step projects the set
of probability measures $\probset$ to a finite vector space using a
(generalized) query operator $\mathbb T$:
\begin{definition}(Query operator)
\label{def:queryop}
 A query operator is a mapping $\mathbb{T} : \mathcal{M}_{\mathbb{P}}(T) \rightarrow \mathcal V \subset \mathbb{R}^\Tdim$ such that for all $\mu, \mu' \in \mathcal{M}_{\mathbb{P}}(T)$ and $\alpha \in [0,1]$,  $\mathbb T (\alpha \mu + (1-\alpha) \mu') = \alpha \mathbb T \mu + (1-\alpha) \mathbb T \mathbb \mu'$. Furthermore, we say that a (nonlinear) operator $\mathbb T^{\dagger}: \mathcal V \to \probset$ is a pesudo-inverse of $\mathbb T$ if $\mathbb T \mathbb T^{\dagger} = I_{\mathcal V}$ is the identity operator.  
\end{definition}




\paragraph{Data sanitization \textit{(2)}:} the second step privatizes
the vector $v=\mathbb T\mu_D$. A standard approach for doing so is the
Laplace mechanism \citep{dwork2006calibrating}, where we set $\nudp =
v + \eta$ with $\eta$ being a Laplace random vector. In this paper we
use the following extension proposed in \citep{xiao2010differential}
and also implicitly used in \citep{boedihardjo2022private}, which
first applies the matrix transform 
\begin{equation}
\label{eq:noiseeq}
    \nudp =  \left[\Phi\left(\Phi^{-1} \begin{bmatrix} \mathbb T\mu_D \\0\end{bmatrix} + \eta\right)\right]_{1:\Tdim},
\end{equation} 
where $\Phi \in \mathbb R^{\Tdim_{\Phi} \times \Tdim_{\Phi}}$ is some
invertible matrix of dimension $\Tdim_{\Phi} \geq \Tdim$ (e.g., the
Haar matrix described in Appendix~\ref{apx:haar} with $\Tdim_{\Phi}=
2^k$ and  $k = \lceil\log_2(\Tdim) \rceil$). We can now show
Lemma~\ref{lm:privacy_phi} which gives an upper bound for the variance
of $\eta$ that is sufficient to guarantee that $\nudp$ is
$\epsilon$-DP. The lemma is a direct consequence of Theorem
3.6 in \citep{gauss_mechanism} 
% and Theorem 1 in \citep{geng2018truncated} (truncated Laplace mechanism) 
with sensitivity
\begin{equation}
    \Delta
    :=\sup_{H(D, D') \leq 1} \left\| \Phi^{-1} \begin{bmatrix}\mathbb{T} \mu_D \\  0 \end{bmatrix}- \Phi^{-1} \begin{bmatrix}\mathbb{T}\mu_{D'}\\0 \end{bmatrix} \right\|_1  \leq \|\Phi^{-1}\|_1 \Delta_{\mathbb T}, 
\end{equation} 
with $\|.\|_1$ the matrix $(1,1)$-norm and the sensitivity of the
operator $\mathbb T$ is defined as follows.
\begin{definition}(Sensitivity of~$\mathbb T$)
\label{def:sensitivity}
 The sensitivity of $\mathbb T$ is the $\ell_1$-distance of the vectors $\mathbb T \mu_D, \mathbb T \mu_{D'}$ when taking the suprenum over all datasets $D, D' \subset   T^{n}$ of size $n$ which differ in at most one point,
 $   \Delta_{\mathbb{T}} = \sup_{H(D, D') \leq 1} \| \mathbb{T}\mu_D - \mathbb{T}\mu_{D'} \|_1.$
% where the , and thus with Hamming distance  $\rho_H$ at most one. 
\end{definition}


% \fy{from what you wrote I expected this lemma to be on the DP-ness of eq. (6) and not the entire pipeline?}

\begin{lemma} \label{lm:privacy_phi} The vector $\nudp$ is
$(\epsilon,0)$-DP for $\eta \sim \left(\mathrm{Lap}\left(
\frac{\|\Phi^{-1}\|_1 \Delta_{\mathbb
T}}{\epsilon}\right)\right)^{\Tdim_{\Phi}}$.
\end{lemma}






\begin{algorithm}[t!]
\caption{Abstract Privacy Preserving Data Generation}\label{alg:mainalgo}
\begin{algorithmic}[1]
\Require Dataset $D$, privacy parameters $\epsilon, \delta$,  query operator $\mathbb{T}$, loss function~$\utilitylossT$ 
\State  $v \gets \mathbb{T} \mu_D$ 
\State construct a $(\epsilon,\delta)$-DP vector $\nudp$ with $v$ as input 
\State optimize $\mu_{\mathrm{opt}} \in \arg\underset{\mu \in \probset}{\min}~~\utilitylossT(\nudp,  \mathbb T \mu)$ 
\State \Return $\mathcal A(D) \gets \mu_{\mathrm{opt}}$
\end{algorithmic}
\end{algorithm}




%\fy{i would write Step 1: bla ... instead of (1)}
\paragraph{Projection onto the span of $\mathcal V$ \textit{(3):}} The
vector $\nudp$ returned in Step 2 is in $\mathbb R^\Tdim$ but not
necessarily in $\mathcal V$. To project it back to $\mathcal V$, Step
3 uses a loss function $\utilitylossT$ defined on $\mathbb
R^\Tdim\times \mathbb R^\Tdim$ dominating the utility loss
$\utilityloss$ as defined below.
\begin{definition}
\label{def:utilityloss} We say that $\utilitylossT: \mathbb R^\Tdim \times \mathbb R^\Tdim \to \mathbb R$ is a loss function (on $\mathbb R^\Tdim$ dominating $\utilityloss$) if for  a pseudo-inverse $\mathbb T^\dagger$ and for all $v, v' \in \mathcal V$, 
\begin{equation}
    \utilityloss(\mathbb T^\dagger v, \mathbb T^\dagger v') \leq \utilitylossT(v, v').
\end{equation}
\end{definition}
% Optimizing the loss function $\mathcal_F$ can be done in two ways:  
% We can now choose a vector $\nudpV \in \mathcal V$ by solving a convex optimization problem and return in line \textit{(4)} a measure $\tilde \mu$ such that $\mathbb T \tilde \mu = \nudpV$. Finally, 
%Note that we can always find a solution for the optimization problem in Step~3 in Algorithm~\ref{alg:mainalgo} by first solving the convex optimization problem $v = \arg\min_{v' \in \mathcal V} \utilitylossT(v', \nudp)$ and then returning $ \mu_{\mathrm{opt}} = \mathbb  T^\dagger  v$.
If $\utilitylossT$ is a loss function, then we can upper bound the utility loss of~Algorithm~\ref{alg:mainalgo} by the following three terms:
\begin{equation}
    \begin{split}
   &\utilityloss(\mu_D, \mathcal A(D)) \\
   &\leq \utilityloss(\mu_D,\mathbb T ^\dagger\mathbb T\mu_D)+\utilityloss(\mathbb T^\dagger\mathbb T\mu_D,\mathbb T^\dagger\mathbb T\algoD)+\utilityloss(\algoD,\mathbb T^\dagger\mathbb T\algoD)\\
   &\leq
   \utilityloss(\mu_D,\mathbb T ^\dagger\mathbb T\mu_D)+\utilitylossT(\mathbb T\mu_D,\mathbb T\algoD)+\utilityloss(\algoD,\mathbb T^\dagger\mathbb T\algoD)\\
   &\leq
   \utilityloss(\mu_D,\mathbb T ^\dagger\mathbb T\mu_D)+\utilitylossT(\mathbb T\mu_D,\nudp)+\utilitylossT(\nudp,\mathbb T\algoD)+\utilityloss(\algoD,\mathbb T^\dagger\mathbb T\algoD)
   \    \label{eq:utilityUBgeneral} \\
   &\leq \underbrace{\utilityloss(\mu_D, \mathbb T^\dagger \mathbb T \mu_D)}_{\text{projection error}} + \underbrace{2~\utilitylossT(\mathbb T \mu_D, \nudp)}_{\text{privacy error}}+\utilityloss( \algoD , \mathbb T^\dagger\mathbb T  \algoD),
   \end{split}
\end{equation}
where in the last line made use of the fact that $\algoD$ is a
solution for the optimization problem in Step 3 in
Algorithm~\ref{alg:mainalgo}.  The first term in the last line
captures the cost of projecting the probability space $\probset$ to
$\mathbb T^\dagger \mathbb T \probset$, while the second term captures
the cost of constructing a private measure on the smaller projected
probability space. Finally, the third term can be upper bounded by the
worst case projection error and is trivially zero when choosing
$\algoD$ such that $\algoD = \mathbb T^\dagger\mathbb T  \algoD$.
Note that doing so indeed does not affect the other terms in the upper
bound since in Step 3 in Algorithm~\ref{alg:mainalgo}, if we replace
$\algoD=\mu_{\mathrm{opt}}$ by $\mathbb T^\dagger\mathbb
T\mu_{\mathrm{opt}}$, it is still a solution to the minimization
problem, given that $\mathbb T\mathbb T^\dagger$ is the identity
operator. 
















\section{Warm-up: recovering the results in \citep{boedihardjo2022private}}
\label{sec:march}
Before stating our main results in~\Cref{sec:mainthm,sec:mainmeasure},
we first show how to instantiate Algorithm~\ref{alg:mainalgo} to
recover the results in \citep{boedihardjo2021privacy}. This
construction will then serve as basis for the rest of this paper. We
refer to Appendix~\ref{apx:almostsure} for almost sure upper bounds
instead of in expectation. 
%While the results in \citep{boedihardjo2022private}
 %only consider to the expected utility loss, a simple extension yields:
\begin{theorem}(Extension of the results in Section~7 in \citep{boedihardjo2022private})
    \label{thm:march}
For any $t >0$ there exists a randomized algorithm $\gA$ that takes a
data set $D \in T^n$ of size $n$ on a metric space $\brace{T, \rho}$
as input and returns a finitely-supported probability measure
$\f{\gA}{\mu_D}$ such that $\gA$ is $\epsilon$-DP and has expected
utility \eqref{eq:utilityloss} over the set $\mathcal{F}$ of all
$1$-Lipschitz continuous functions at most 
\begin{equation*}
\mathbb E~\f{\utilityloss}{\mu_D, \f{\gA}{D}} \leq  \discdelta  + \frac{128\sqrt{2}\left(\ceil{\log_2\f{N}{T,\rho,\discdelta}} +1\right)^{3/2} }{n \epsilon}\int_{\discdelta/2}^{\f{\mathrm{diam}}{T}/2}\f{N}{T,\rho,x}dx.
\end{equation*}
\end{theorem}
\paragraph{Proof of Theorem~\ref{thm:march}} The proof consists of
 three parts, where we first construct a query operator $\mathbb T$
 (Definition~\ref{def:queryop}), a loss function $\utilitylossT$
 (Definition~\ref{def:utilityloss}), and then derive an upper bound
 for the utility loss using Equation~\eqref{eq:defofHfull}.

 \paragraph{Construction of the query operator $\mathbb T$, the
 pseudo-inverse $\mathbb T^\dagger$ and the operator $\mathbb
 D_{T_\Tdim}$:} Let $\Tdim= N(\T, \rho,\discdelta)$ be the covering
 number of $\T$ and let $T_\Tdim$ be the centers of any minimal
 $t$-covering of $\T$. Furthermore, let $\mathbb D_{T_\Tdim} :
 \measure(\T) \to \measure(T_\Tdim)\subset \measure (\T)$ be the
 projection operator which constructs a probability measure on
 $T_\Tdim$ by dividing the space $\T$ into $m$ disjoint measurable
 neighborhoods around the points in $T_\Tdim$ of diameter at most
 $t$.
 Given any indexing of the elements in $T_\Tdim$, we can
 straightforwardly define a bijection from $\measure(T_\Tdim)$ to the
 probability simplex $\mathcal V = \{z \in \mathbb R^\Tdim: \|z\|_1
 =1, z_i \geq 0\}$ and thus complete the construction of the operator
 $\mathbb T$ (see Definition~\ref{def:queryop}). Furthermore, let the
 pseudo-inverse $\mathbb T^\dagger: \mathcal V \to \measure(T_\Tdim)
 \subset \probset$ be the operator such that~$\mathbb T^\dagger
 \mathbb T = \mathbb D_{T_\Tdim}$. 

To simplify the following analysis, we now describe how to choose a
particular indexing of the elements in $T_\Tdim$ based on the analysis
in~\citet{boedihardjo2022private}.  Proposition 6.5 and Equation (7.4)
in \citep{boedihardjo2022private} together guarantee the existence of
a finite set $\Omega =\{w_1, \cdots, w_\Tdim\} \subset [0,L]$  as well
as a $1$-Lipschitz (w.r.t.~$\rho$) bijection $f: ~\Omega \to T_\Tdim$
with
\begin{equation}
    L =  64 \int_{t/2}^{\diam(T)/2} N(T, \rho, x) dx.
\end{equation}
  Note that w.l.o.g.~we can assume that $w_i \leq w_{i+1}$
 which thereby implicitly induces a Markovian path on $T_\Tdim$ of length at most $L$. We can now define the indexing of the elements in $T_\Tdim$ by $z_i = f(w_i)$, 
  which allows us to  complete the construction of the operator $\mathbb T$.
 


\paragraph{Construction of the loss function $\utilitylossT$:} 
One of the key ideas of~\citet{boedihardjo2022private} is to reduce the the problem of constructing a private measure on $T$ to that of constructing a private measure on an interval on $\mathbb R$. This is done via the bijection $f$ introduced in the previous paragraph. Along these lines, we now show how we can make use of the bijection $f$ to construct a loss function $\utilitylossT$ satisfying the conditions in Definition~\ref{def:utilityloss}. 

If $\mu_{T_\Tdim}\in\measure(T_\Tdim)$, then let $\mu_{T_\Tdim,f}$ be the push-forward measure of  $\mu_{T_\Tdim} \in \measure(T_\Tdim)$, i.e. the measure on $\measure(\Omega)$ such that for any $A \subset \Omega$,
$\mu_{T_\Tdim,f}(A) = \mu_{T_\Tdim}(f(A))$. Since $f$ is a $1$-Lipschitz continuous function, the Wasserstein distance of any two measures $\mu_{T_\Tdim}, \mu_{T_\Tdim}' \in \measure(T_\Tdim)$ is upper bounded by
\begin{equation}
\begin{split}
\label{eq:ubHfull}
  \utilityloss(\mu_{T_\Tdim}, \mu_{T_\Tdim}') &= W_1(\mu_{T_\Tdim}, \mu_{T_\Tdim}') \leq W_1(\mu_{T_\Tdim,f}, \mu_{T_\Tdim,f}') \\
  &=
% \end{equation}
% One of the key insights in the analysis in the paper \citep{boedihardjo2022private} is now to use the following identity by 
% \begin{equation}
      \| F_{\mu_{T_\Tdim,f}} - F_{\mu_{T_\Tdim,f}'}\|_{L^1(\mathbb R)} \\&
      =\sum_{j=1}^\Tdim (w_{j+1} - w_j) \left\vert \sum_{i=1}^j (\mu_{T_\Tdim}(f^{-1}(w_{i})) -  \mu_{T_\Tdim}'(f^{-1}(w_{i})))\right\vert \\&
      =\sum_{j=1}^\Tdim (w_{j+1} - w_j) \left\vert \sum_{i=1}^j (v_i -  v'_i)\right\vert 
     \end{split}
      \end{equation}
where the second equality follows from the identity
in~\citet{vallender74}, $F_{\mu_{T_\Tdim,f}}$ is the cumulative distribution
function of the measure $\mu_{T_\Tdim,f}$, and we use the notation $v
= \mathbb T \mu_{T_\Tdim}$, $v' = \mathbb T \mu_{T_\Tdim}'$, and
$w_{\Tdim+1}= L$.  Using the RHS of~\Cref{eq:ubHfull} to define the
utility loss function $\utilitylossT$ on $\mathbb R^\Tdim$
\begin{equation}
   \utilitylossT(v, v') :=\sum_{j=1}^\Tdim (w_{j+1} - w_j) \left\vert \sum_{i=1}^j (v_i -  v'_i)\right\vert,
         \label{eq:defofHfull}
\end{equation}
we have
$\utilityloss(\mu_{T_\Tdim},\mu_{T_\Tdim}')\leq\utilitylossT(\mathbb
T\mu_{T_\Tdim},\mathbb T\mu_{T_\Tdim}')$ for all
$\mu_{T_\Tdim},\mu_{T_\Tdim}'\in\measure(T_\Tdim)$.
%Clearly, $\utilitylossT$ is a convex function and by the construction of $\mathbb T$ and $\mathbb T^\dagger$, we have that for any pair of  measures $\mu, \mu' \in \measure(\T)$, $\utilityloss(\mathbb T^\dagger \mathbb T \mu, \mathbb T^\dagger \mathbb T \mu') = W_1(\mathbb T^\dagger \mathbb T \mu, \mathbb T^\dagger \mathbb T \mu') \leq \utilitylossT(\mathbb T \mu, \mathbb T \mu')$.
Hence, we conclude that $\utilitylossT$ satisfies the conditions in Definition~\ref{def:utilityloss}. 


\paragraph{Upper bound for the utility loss $\utilityloss$:} Finally, we can prove Theorem~\ref{thm:march} by upper bounding the utility loss using Equation~\eqref{eq:utilityloss}.
Note that we can always choose $\mathcal A(D)$ such that $\utilityloss( \algoD , \mathbb T^\dagger\mathbb T  \algoD) =0$. Thus, we only need to bound the projection error and privacy error terms in Equation~\eqref{eq:utilityloss}. First, the projection error term in
Equation~\eqref{eq:utilityUBgeneral} can be upper bounded by
 \begin{equation}
     \sup_{\mu \in \probset} \utilityloss(\mu, \mathbb T^\dagger \mathbb T \mu ) =  \sup_{\mu \in \probset} W_1(\mu, \mathbb T^\dagger \mathbb T \mu ) = \sup_{\mu \in \probset}  W_1(\mu, \mathbb D_{T_\Tdim} \mu )\leq \discdelta, 
 \end{equation}
 which is a consequence of the fact that $\mathbb D_{T_\Tdim}$ moves every point mass at most distance  $\discdelta$.  
 
Next, we bound the privacy error in Equation~\eqref{eq:utilityUBgeneral}. To do so, we first need to choose the matrix $\Phi$ in Equation~\eqref{eq:noiseeq}. As first suggested in \citep{xiao2010differential} and also in \citep{boedihardjo2022private}, we can choose $\Phi =(\ceil{\log_2(\Tdim)} + 1) M_{\ceil{\log_2(\Tdim)}}$ where
 $M_k$ is the $k$-th Haar Matrix (see Appendix~\ref{apx:haar}) and then apply the Laplace mechanism as in Lemma~\ref{lm:privacy_phi}. 
% construct the DP vector $\nudp$ in Step 2 in Algorithm~\ref{alg:mainalgo} by first applying the Haar matrix transformation as in Equation~\eqref{eq:noiseeq} with 
 % or the truncated Laplace mechanism which guarantees that $\mathcal A$ is $(\epsilon, \delta)$-DP, respectively. 
% Using this choice of $\Phi$, we can upper bounding the expected privacy error
 % term  $ \mathbb E~\utilitylossT(\mathbb T \mu_D , \nudp)$. 
 % Equation~\eqref{eq:utilityUBgeneral}\red{this is a bit confusing as
 % it is not clear which proof you are referring to. Maybe in the
 % beginnning we should state we are going to bound the three terms, the
 % first followins from ... (i..e 13) and the next by bounding the
 % privacy loss etc. Otherwise this paragraph is not very clear what it
 % is trying to achieve}.
 First note that $
 \Delta_{\mathbb T} \leq \frac{2}{n}$ where $\Delta_{\mathbb T}$ is
 defined in Definition \ref{def:sensitivity}. Indeed, the vectors
 $\mathbb T\mu_D$ and $\mathbb T\mu_{D'}$ are representations for the
 discretized measures $\mathbb D_{T_\Tdim} \mu_D$ and $\mathbb
 D_{T_\Tdim} \mu_{D'}$, which differ at most in one point. By Lemma~\ref{lm:privacy_phi} we therefore need to draw 
${\eta  \sim \left(\text{Lap}\left(\frac{2\|\Phi^{-1}\|_1}{n \epsilon} \right)\right)^{m_{\Phi}}}$. A straightforward calculation then yields the following upper bound for the privacy error in Equation~\eqref{eq:utilityUBgeneral}:
% \begin{lemma} \label{thm:utility_phi}
%     $\sup_{v \in \mathcal V} \mathbb E~\utilitylossT(v,v + \Phi \eta)  \leq \frac{2\|\Phi^{-1}\|_1 L}{n \epsilon} \cdot \max_{i = 1}^\Tdim \| \sum_{j = 1}^i \Phi_j \|_2$ 
% \end{lemma}
        \begin{equation}
        \begin{split}
          \mathbb E ~&\utilitylossT(\mathbb T \mu_D, \nudp) =  \mathbb E ~\utilitylossT(\mathbb T \mu_D, \mathbb T \mu_D + [\Phi \eta]_{1:\Tdim}) \\
          &=\sum_{j=1}^\Tdim (w_{j+1} - w_j) \mathbb E_{\eta \sim \left(\text{Lap}\left(\frac{2 \|\Phi^{-1}\|_1}{n \epsilon} \right)\right)^{\Tdim_{\Phi}}}\left\vert \sum_{i=1}^j (\Phi \eta)_i\right\vert  \\
      &\stackrel{(\text{Jensen})}{\le}  L \max_{j = 1}^\Tdim  \mean{ \text{std} \left(\sum_{i = 1}^j (\Phi \eta)_i \right)}{\eta \sim \left(\text{Lap}\left(\frac{2 \|\Phi^{-1}\|_1}{n \epsilon} \right)\right)^{\Tdim_{\Phi}}}   = \frac{2\sqrt{2}L \|\Phi^{-1}\|_1}{n \epsilon} \cdot \max_{j = 1}^\Tdim \left \| \sum_{i = 1}^j \Phi_i \right \|_2, \label{eq:marchboundexp}
        \end{split}
        \end{equation}
 where $\Phi_i$ is the i-th row of $\Phi$. 
We then obtain the desired  upper bounds when applying Lemma~\ref{lm:haar_properties} in Appendix~\ref{apx:haar}. 

 


% In this last paragraph we discuss how to obtain an upper bound for the worst case expected 


% Finally, we can complete the proof with the following upper bound on the 
%  % We can then apply the Kantorovich-Rubinstein duality Theorem, which states that $\utilityloss = W_1$ and thus















==> sections/old_sections/Section3_analysis.tex <==
\section{Guarantees for sparse Lipschitz continuous functions}
\label{sec:mainthm}
We now turn to our first abstract main result of this paper, where we show fast rates for the utility loss over all sparse Lipschitz continuous functions. 
Generally, we can ask for an algorithm $\mathcal A$, taking a data set $D \in T^n$ on some measurable space  $(T, \mathcal B)$ as input, to achieve a small utility loss over a function class
\begin{equation}
\label{eq:funcclasssparse}
    \mathcal F = \bigcup_{i=1}^K \mathcal F_{(i)} :=  \bigcup_{i=1}^K\{f_{(i)}\circ \projectfunci\vert f_{(i)}~\text{is 1-Lipschitz~w.r.t.~} \rho_{(i)}\},
\end{equation}
with $(T_{(i)}, \rho_{(i)})_{i=1}^K$ being some set of metric spaces and surjective measurable functions $\projectfunci : T \to T_{(i)}$ serving as ``projections'' of $T$ to $T_{(i)}$. We assume that the push-forward $\sigma$-algebras generated by $h_{(i)}$ coincide with the $\sigma$-algebras generated by $\rho_{(i)}$ on $T_{(i)}$.

Further, let $\projectopi: \probset \to \measure(T_{(i)})$ be the
push-forward operators such that $\projectopi \mu \in
\measure(T_{(i)})$ are the induced measures by $\projectfunci$.
Analogous to Equation~\eqref{eq:wassersteinsparse}, by the
Kantorovich-Rubinstein Duality Theorem~\citep{Villani2008OptimalTO},
the utility loss (see Equation~\eqref{eq:utilityloss}) is exactly the
maximum of the Wasserstein distances w.r.t. the metrics $\rho_{(i)}$,
\begin{equation}
\label{eq:Wassersteinsparse}
    \utilityloss(\mu, \tilde \mu) = \max_{i\in\{1, \cdots, K\}} W_1(\projectopi \mu,  \projectopi \tilde \mu).
\end{equation}
To give an example, in the context of Corollary~\ref{cor:rates}, we have $K ={d \choose s}$ and $T_{(i)} = [0,1]^s$  are the $s$-sparse marginals of $T$ with $\rho_{(i)}(x,y) = \|x-y\|_{\infty}$. Furthermore, $h_{(i)}$ are the functions projecting  $x\in [0,1]^d$ to the corresponding $s$-dimensional subspaces and $\projectopi \mu$ are the marginal measures of $\mu$ on the corresponding $s$-dimensional subspaces. 








We now turn to our main result, Theorem~\ref{thm:mainthm}, which
provides a general upper bound for the utility loss over the function
class $\mathcal F$. When $K=1$ we can directly obtain the upper bounds
in Theorem~\ref{thm:mainthm} from the results in
\citep{boedihardjo2022private}, restated in Theorem~\ref{thm:march} in
Section~\ref{sec:march}. The main technical contribution of this paper
is to show that the price to pay if $K>1$ is at most linear in $K$
(plus a logarithmic factor if $\delta =0$).
% the case where $\mathcal F$ is the set of all $1$-Lipschitz continuous functions on a metric space $(T, \rho)$. 
% $T$ is, 
% the rates for the utility loss are generally expected to be slow unless $T$ is a "low-dimensional" space (See Section~9 in \citep{boedihardjo2022private}). 
% In this section, we show how the framework presented in Algorithm~\ref{alg:mainalgo} allows us to straight forwardly generalize Theorem~\ref{thm:march} to the case

% \red{rewrite !}
% We now present an upper bound for the utility loss for the function class 
% In particular, we given an explicit example where $\mathcal F$ is the set of sparse $1$-Lipschitz continuous functions on the hypercube and  support the upper bound with a matching lower bound. 
% We then discuss practical implications in Section~\red{bla}. 
% In its general form, we let 


\begin{theorem}\label{thm:mainthm}
For the setting described in Section~\ref{sec:mainthm}, there exists a
universal constant $c >0$ and a randomized algorithm $\gA$ that takes
a data set  $D \in T^n$ of size $n$  as input and returns a
finitely-supported measure $\f{\gA}{\mu_D} \in \probset$ such that
$\gA$ is $\epsilon$-DP private and has expected utility
loss~\eqref{eq:utilityloss} over the function class $\mathcal F$,
defined in Equation~\eqref{eq:funcclasssparse}, at most 
\begin{equation} 
\begin{split}
\label{eq:eq1mainthm}
\mathbb E&~\f{\utilityloss}{\mu_D, \f{\gA}{D}} \leq t \\
&+ c  K \bigg[\max_{i\in\{1, \cdots, K\}} \left(\ceil{\log_2\f{N}{T_{(i)},\rho_{(i)},t}} + 1 + \log(K)\right)^2 
\int_{t/2}^{\f{\mathrm{diam}}{T_{(i)}}/2}\f{N}{T_{(i)},\rho_{(i)},x}dx\bigg].
\end{split}
\end{equation}
\end{theorem}
We refer to Appendix~\ref{apx:almostsure} for almost sure upper bounds instead of in expectation.
The proof closely follows the proof of Theorem~\ref{thm:march}.  We therefore only present a proof sketch highlighting the changes in the main text and refer the reader to Appendix~\ref{apx:main} for the full proof of the theorem.
%A the full proof of Theorem~\ref{thm:mainthm} in 
%based on the following proof sketch:
\paragraph{Proof of Theorem~\ref{thm:mainthm}}
%When $K=1$ we the result directly follows Theorem~\ref{thm:march} in Section~\ref{sec:march}. 
% As we show in the proof, we can extend the result for the case where
% $K=1$ in Theorem~\ref{thm:march} in Section~\ref{sec:march} to the
% case of $K>1$ when constructing a query operator $\mathbb T$ (see
% Definition~\ref{def:queryop}) with $\Tdim = \sum_i \Tdim_{(i)}$ by
% simply  stacking the operators $\mathbb T_{(i)} \circ  \projectopi
% :\measure(T) \to \mathbb R^{\Tdim_{(i)}}$ where $\mathbb T_{(i)}$ are
% the query operators described in Section~\ref{sec:march} for the
% metric spaces $(T_{(i)}, \rho_{(i)})$.  It is then straight forward to
% verify that for any pseudo-inverse, the projection error
% $\utilityloss(\mu_D, \mathbb T^\dagger \mathbb T \mu_D) \leq t$
% \red{we should remove \(\leq t\) from here ?} from
% Equation~\eqref{eq:utilityUBgeneral} is upper bounded by $t$.

% \red{Can we change this paragraph to following}

As we show in the proof, we can extend the result for the case
where $K=1$~(in Theorem~\ref{thm:march} in Section~\ref{sec:march}) to
the case of $K>1$ by changing the query operator $\mathbb T$ from
Definition~\ref{def:queryop}. We construct \(\mathbb{T}\) with $\Tdim
= \sum_i \Tdim_{(i)}$, by simply stacking the operators $\mathbb
T_{(i)} \circ \projectopi :\measure(T) \to \mathbb R^{\Tdim_{(i)}}$
where $\mathbb T_{(i)}$ are the query operators described in
Section~\ref{sec:march} for the metric spaces $(T_{(i)}, \rho_{(i)})$.
It is then straight forward to verify that for any pseudo-inverse, the
projection error $\utilityloss(\mu_D, \mathbb T^\dagger \mathbb T
\mu_D)$ from
Equation~\eqref{eq:utilityUBgeneral} is upper bounded by $t$.

In Step 2 of Algorithm~\ref{alg:mainalgo}, we apply the transformed
Laplace mechanism to every block $\nu_{(i)} \in \mathbb
R^{\Tdim_{(i)}}$ as described in the proof Theorem~\ref{thm:march}.
However, this requires increasing the sensitivity to $\Delta_{\mathbb
T} \leq \frac{2K}{n}$ due to the increased total number of
measurements. Since the utility loss function $\utilityloss$ is simply
the maximum over the Wasserstein distances over the projected measures
of every subspace $T_{(i)}$ (see
Equation~\eqref{eq:Wassersteinsparse}), we can define the loss
function $\utilitylossT$ dominating the utility loss $\utilityloss$
(see Definition~\ref{def:utilityloss}) to be the maximum loss
$\utilitylossT(\nu, \nu') = \max_{i\in\{1, \cdots, K\}}
~\utilitylossTi(\nu_{(i)}, \nu_{(i)}')$  where $\nu_{(i)} \in \mathbb
R^{\Tdim_{(i)}}$ is the $i$-th block of the vector $\nu \in \mathbb
R^\Tdim$ and $\utilitylossTi$ is the corresponding loss function as
constructed in the proof of Theorem~\ref{thm:march}. We then obtain
the desired result when bounding the privacy error term
$\utilitylossT(\mathbb T \mu_D, \nudp)$ in
Equation~\eqref{eq:utilityUBgeneral} using
Lemma~\ref{lm:mainappendix}. 













% We can then apply the same analysis as des








%\paragraph{Construction of $\mathbb T$, $\utilitylossT$ and $\Phi$:}




% Clearly, the conditions in Definition~\ref{def:queryop} and \ref{def:utilityloss} are satisfied. 



% We present a proof for the main result in Section~\ref{subsec:proofmainthm} when $K>1$, where we straight forwardly extend the construction presented in Section~\ref{sec:march}. 

% and first now as the proof of Corollary~\ref{cor:rates}.

\paragraph{Proof of Corollary~\ref{cor:rates}}
Finally, we discuss how Theorem~\ref{thm:mainthm} implies Corollary~\ref{cor:rates}. We recall that in this case,  $T_{(i)} =[0,1]^s$ and $\rho_{(i)} = \|. \|_{\infty}$, and thus, for any $k \in \mathbb N_{>0}$, we can simply upper bound the covering numbers by $N(T_{(i)}, \|.\|_{\infty},t) \leq k^s.
$ with $t=1/2k$.
Plugging this upper bound into Equation~\eqref{eq:eq1mainthm} in Theorem~\ref{thm:mainthm} and using that  ${d \choose s} \asymp d^s$, we obtain 
 $   \mathbb E ~\utilityloss(\mu_D, \algoD) \lesssim_s \frac{1}{2k} + \frac{d^s \log(k)^{3/2}}{n \epsilon} k^{s-1}$, 
 where $\lesssim_s$ is hiding constants depending on $s$. We obtain the desired result when optimizing over $k$. 
%and repeating the same argument for Equation~\eqref{eq:eq2mainthm}. 



% f Algorithm~\ref{alg:mainalgo} (see Section~\ref{sec:algo}) in Section~\ref{sec:march}, and then generalize the proof to the case where Section~\ref{subsec:proofmainthm}.















% \begin{theorem}(Theorem bla in \citep{boedihardjo2022private})
%     \label{thm:mainthm}
%   There exists a randomized algorithm $\gA$ that takes an empirical measure $\mu_D$ with $D \in T^n$ on $\brace{T, \rho}$ as input and returns a finitely-supported probability measure $\f{\gA}{\mu_D}$ on $\brace{T, \rho}$ such that $\gA$ is $\epsilon$-DP private and has utility\footnote{The explicit constants are derived in Section~where. Theorem~bla in \citep{boedihardjo2022private} does not provide the explicit constants. }
% \begin{equation*}
% \f{U_s}{\mu_D, \f{\gA}{D}} \leq 2\delta + \sup_{S \subset \{1, \cdots, d\}, \vert S \vert = s}\frac{4\mathrm{diam}(T_S)\sqrt{2}}{n \epsilon}\log^{3/2}\brace{\f{\gN}{T_S,\rho_S,\delta}}\int_{\delta}^{\f{\mathrm{diam}}{T_S}}\f{\gN}{T_S,\rho,x}dx.
% \end{equation*}
% for any $\delta \geq 0$ where $\matchal N(T,\rho,\delta)$ is the $\delta$-covering number and $\diam(T)$ the diameter of~$T$.
% \end{theorem}

% We now present our main result which is a generalization of Theorem~\red{which one} in \citep{boedihardjo2022private}. 









% We choose $\mathcal F_s $ to be the set of all 1-Lipschitz continuous functions that only depend on $s$-dimensions. 
% Let $(T,\rho)$ be any metric space with $T \subset \mathbb R^d$ and for every $S \subset \{1,\cdots, d\}$, let  $(T_{\mathcal S},\rho)$ be the metric space obtained when projecting $T$ onto the the dimensions indexed by $S$. 




















% Indeed, by construction we have that for any $i \in \{1, \cdots, K\}$ and measures ${\mu_{(i)}, \mu_{(i)}' \in \measure(T_{(i)})}$ that 
% \begin{equation}
%   \mathbb T_{(i)} \mu_{(i)} = \mathbb T_{(i)} \mu_{(i)}' \implies W_1(\mu_{(i)} , \mu_{(i)}' ) \leq t. 





% Furthermore, we will make use of the fact that 
% \begin{equation}
%     U_{\mathcal F}(\mu, \mu') = \max_{i\in\{1, \cdots, K\}}~ W_1(\mathbb \utilitylossTi \mu, \mathbb \utilitylossTi \mu')
% \end{equation}
% We now show how we can straight forwardly extend  the construction to the case where $K>1$ and then upper bound the utility loss $\utilityloss(\mu_D, \algoD)$ using the upper bound in Equation~\eqref{eq:utilityUBgeneral}. 


% The proof follows the same structure as in Section~\ref{Sec:march}. 







% \paragraph{Construction of the loss function $\utilitylossT$:}
% Let $\nu_{(i)} \in \mathbb R^{N_{(i)}}$ be the $i$-th component of the vector $\nu \in \mathbb R^N$ and define
% $\utilitylossT(\nu, \nu') = \max_{i\in\{1, \cdots, K\}} ~\utilitylossTi(\nu_{(i)}, \nu_{(i)}')$ . 














% which is also the part in this proof which differs from the proofs in \citep{boedihardjo2022private}. 









==> sections/old_sections/Section4_example.tex <==



\section{Guarantees for ``low-dimensional" data}
\label{sec:mainmeasure}
In Section~\ref{sec:mainthm}, we improved the rates for the utility
loss $\utilityloss$ (see Equation~\eqref{eq:utilityloss}) over all
Lipschitz continuous functions in Equation~\eqref{eq:utilityloss} by
restricting the set of functions $\mathcal F$ to $s$-sparse functions.
As a second abstract main result in this paper, we present fast rates
for the utility loss over all Lipschitz continuous functions but
assuming that the data lies on a ``low-dimensional subspace'', in the
sense described below. 
% We again first discuss the example where the underlying space is the $d$-dimensional Hypercube $T =  [0,1]^d$.
% Let
% $ T_k = \{ 1/2k, \cdots , (2k-1)/2k\}^d$
% be the centers of a minimal $1/2k$-covering of $T$ of size $\Tdim =k^d$. For any data set $D$ we define the pseudo-dimension of the data:
% \begin{definition}(pseudo-dimension of the data)
% For any constant $c$ and any data set $D$ let $s_c(D) \in [0,d]$  be the smallest number such that for all $k\geq 1$, $D$ is contained in at most $c k^s$ $\ell_{\infty}$-balls of radius   $1/2k$ with centers in $T_k$.
% \end{definition}
% As a corollary of  Theorem~\ref{thm:mainthmmeasure} in this section, we will show the following formal statement for Equation~\eqref{eq:ratesmeasure}, demonstrating that we can achieve significantly faster rates when the data has small pseudo-dimension:
% \begin{corollary}(of Theorem~\ref{thm:mainthmmeasure})
% \label{cor:ratesmeasure}
% Let $\mathcal F$ be the set of all $1$-Lipschtiz continuous functions on $[0,1]^d$ with respect to the $\ell_{\infty}$-distance metric. 
% There exists an $\epsilon$-DP algorithm $\mathcal A$ such that Equation~\eqref{eq:ratesmeasure} holds
% with $s= s_c(D)\in[0,d]$ is the pseudo dimension of the data $D$ for some unviersal constant $c$.
% % Furthermore, there exists an $(\epsilon,\delta)$-DP algorithm $\mathcal A$ such that almost surely, 
% % \begin{equation}
% % \label{eq:ubfull}
% %      \utilityloss(\mu_D, \algoD) \lesssim_{s_c(D)} \left( \frac{d\log(\epsilon n) \log(1 + \frac{e^\epsilon -1}{2 \delta})}{n \epsilon}\right)^{1/(s_c(D)+1)}.
% % \end{equation}
% \end{corollary}
% The proof of the corollary follows from exactly same argument as the proof of Corollary~\ref{cor:rates} when using Theorem~\ref{thm:mainthmmeasure} below.
% The algorithm in Corollary~\ref{cor:ratesmeasure} ``adapts'' to the ``sparsity'' $s_c(D)$ of the data and
% does not make use of any oracle knowledge of  $s_c(D)$. In the worst case when $s_c(D) = d$ we obtain a rate of order $n^{-1/(d+1)}$, ignoring logarithmic factors. When comparing with the rate in Equation~\eqref{eq:ubfull} of order $n^{-1/d}$, we see that an additional $+1$ term appears in the exponent, which is the price to pay for the adaptivity.  
For any $t > 0$ and metric space space $\brace{T, \rho}$, fix a
minimal $t$-covering $T_\Tdim$ of size $N(T, \rho, t)$ and let
$\discfunct: T \to  T_\Tdim$ be any measurable discretization map such
that for any point $x \in T$, $\rho(\discfunct(x), x) \leq
t$. Further, let $\vert q_t(D)\vert$ be the size of the support of $q_t(D)$ (which captures the ``sparsity'' of the subspace the data is lying on).
% \red{Mention here once again how q represents the sparsity}%Furthermore, for any data set $D \in T^n$ let $ \vert
% \text{supp}_{f,t}(D)\vert \leq \min(n, \Tdim)$ be the size of the
% support of the set $f(D)$.
\begin{theorem}
    \label{thm:mainthmmeasure}
In the setting described above, there exists a randomized algorithm
$\gA$ that takes a data set $D \in T^n$ of size $n$  as input on a
metric space $\brace{T, \rho}$ and returns a finitely-supported
probability measure $\f{\gA}{\mu_D}$ on $\brace{T, \rho}$ such that
$\gA$ is $\epsilon$-DP private and has expected utility loss
\eqref{eq:utilityloss} over the set of all $1$-Lipschitz continuous
functions with respect to $\rho$ at most: 
\begin{equation}
\label{eq:ubmeasure}
\mathbb E~\f{\utilityloss}{\mu_D, \f{\gA}{D}} \leq \discdelta +  \frac{64~\mathrm{diam}(T) \log(\Tdim+1)}{n \epsilon}  ~\vert \discfunct(D)\vert 
\end{equation}
% Furthermore, for any $\delta \geq 0$ there exists an $(\epsilon, \delta)$-DP algorithm such that almost surely
% \begin{equation*}
% \f{\utilityloss}{\mu_D, \f{\gA}{D}} \leq \discdelta + \frac{64~\mathrm{diam}(T) \log(\Tdim+1)}{n \epsilon}   \log\left(1 + \frac{e^\epsilon - 1}{2\delta}\right) ~\vert \mathrm{supp}_{f,t}(D)\vert
% \end{equation*}
\end{theorem}
\noindent We refer to Appendix~\ref{apx:almostsure} for almost sure
upper bounds instead of in expectation.

\paragraph{Proof of Theorem~\ref{thm:mainthmmeasure}} As in the proof
of Theorem~\ref{thm:march}, let $\mathbb D_{T_\Tdim} : \probset \to
\measure(T_\Tdim)$ be any projection operator and let $\mathbb T\mu
\in \mathcal V = \{z \in \mathbb R^\Tdim: \|z\|_1 =1, z_i \geq 0\} $
be the vector representing the measure $\mathbb D_{T_{\Tdim}} \mu$.
Unlike in the the proof of Theorem~\ref{thm:march}, we can choose any
random indexing of the elements in $T_\Tdim$ to represent the vector
$\mathbb T \mu$. 

\paragraph{Data sanitization, Step 2 in Algorithm~\ref{alg:mainalgo}:}
The main idea of the proof is now to make use of the fact that the
vector $\mu$ is $\vert \discfunct(D)\vert$-sparse. Thus, in Step 2 in
Algorithm~\ref{alg:mainalgo} we can make use of results on the DP
release of sparse histograms (see e.g.,
Section~\ref{sec:relatedwork}). Since we do not optimize  for the
computational run-time complexity in this result (see
Section~\ref{sec:experiment} for a discussion on that topic), a simple
way to construct a sparse private variant of $v$ is: first apply the
standard Laplace mechanism (with $\Phi=I_\Tdim$) to obtain a
differential private copy of $ \tilde{v}_{\text{DP}} = v + \eta$  of
$v$ with $\eta$ as in Lemma~\ref{lm:privacy_phi} and then solve the
convex optimization problem
\begin{equation}
    \nudp = \arg\min_{v'} \|v' - \tilde{v}_{\text{DP}} \|_2 \quad \text{s.t.}~\|v'\|_1 \leq 1
\end{equation}
Standard results for the constrained $\ell_1$-norm ERM solution (see e.g., Theorem 7.13 in \cite{wainwright2019high}) then yield the following upper bound on the $\ell_1$-error $ \|\nudp - v \|_1 \leq 16 \vert\discfunct(D)\vert   \|\eta\|_{\infty}$.


\paragraph{Construction of the loss function $\utilitylossT$ and upper bound for the utility loss $\utilityloss$:}
The proofs of  Theorem~\ref{thm:march} and \ref{thm:mainthm} strongly
rely on the correlated noise induced by the choice of $\Phi$ in
Equation \eqref{eq:noiseeq} together with the loss function
$\utilitylossT$ constructed in the proof of  Theorem~\ref{thm:march}.
Because of the construction of $\nudp$ in this proof %\red{maybe say
%the reason more explicityly, it is not constructed but is the solution
%of an opt problem}
we can no longer make use of the mentioned analysis,
which also explains why the rate in the upper bound in
Corollary~\ref{cor:rates} does not recover the rate in the upper bound
in Equation~\eqref{eq:ubfull} when $s =d$. Instead, a simple way to
construct the loss function $ \utilitylossT$ (see
Definition~\ref{def:utilityloss}) is to naturally extend the operator
$\mathbb T^\dagger$ to inputs in $\mathbb R^\Tdim$ returning signed
measures on $T_\Tdim$ and define
\begin{equation}
\label{eq:lossmeasure}
 \utilitylossT(v, v') := \sup_{f \in \mathcal F; f(0) =0} \left \vert \sum_{z_i \in T_\Tdim} f(z_i) ~ (\mathbb T^\dagger v)(\{z_i\}) - \sum_{z_i \in T_\Tdim} f(z_i) ~(\mathbb T^\dagger v')(\{z_i\})\right \vert.
\end{equation}
We remark that the loss function in
Equation~\eqref{eq:lossmeasure} has also been used in the concurrent
work \citep{Yiyun23} to obtain sharper rates than in
Equation~\eqref{eq:ubfull} without logarithmic factors.
Restricting $f(0) = 0$ is crucial since without this assumption, Equation~\eqref{eq:lossmeasure} is infinite if $\|v\|_1 \neq \|v'\|_1$. 
Note however that restricting $f(0)=0$ still results in a valid loss function $\utilitylossT$ dominating $\utilityloss$. Indeed, for any function $f \in \mathcal F$, constant $c\in \mathbb R$ and probability measures $\mu, \mu' \in \measure(T)$ we have $   \vert  \int f d\mu  - \int f d\mu'\vert =   \vert  \int (f+c) d\mu  - \int (f+c) d\mu'\vert$. 

\paragraph{Upper bound for the utility loss $\utilityloss$:} Recall
from the proof of Theorem~\ref{thm:march} that the projection error
$\utilityloss(\mu_D, \mathbb T^\dagger \mathbb T \mu_D) \leq t$ from
Equation~\eqref{eq:utilityUBgeneral} is upper bounded by $t$.  We can
upper bound the (expected) privacy error term  $ \utilitylossT(\mathbb
T \mu_D , \nudp)$ in Equation~\eqref{eq:utilityUBgeneral} by:
\begin{equation}
\begin{split}
    \utilitylossT(\mathbb T \mu_D, \nudp) &\leq \sup_{f\in F; f(0) = 0}  \sum_{z_i \in T_\Tdim} \vert f(z_i) (v_{\mathrm{DP},i} - v_i)\vert \overset{\mathrm{\text{H\"older}}}{\leq} \sup_{f\in F; f(0) = 0} \|f\|_{L_{\infty}} \|\nudp - v\|_1 \\
     &\leq \mathrm{diam}(T) ~16 ~\vert \discfunct(D)\vert ~ 
    \|\eta\|_{\infty}.
    \label{eq:finalubmainmeasure}
    \end{split}
\end{equation}
We then obtain the desired result when using the upper bound $\mathbb E~\|\eta\|_{\infty} \leq \frac{4}{n \epsilon} \log(\Tdim+1)$ where we used Example 2.19 in \citep{wainwright2019high} in the last line and the fact that  $\|\eta\|_{\psi_1} =2$ for $\eta \sim \mathrm{Lap}(1)$. 



% In total, the algorithm is therefore $\epsilon$-DP, as desired. 



















\section{Practical aspects and future work}
\label{sec:experiment}
As demonstrated in Corollary~\ref{cor:rates} and
\ref{cor:ratesmeasure}, even for data sets of moderate dimensions and
limited number of data points $n$, we can construct a private data set
with small expected utility loss when $s$ is a small integer.  This
motivates the question of practically efficient algorithms. In this
discussion, we focus on the instantiation of
Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthm}, and only
mention that efficient implementations for the  instantiation of
Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthmmeasure} have
been proposed in the concurrent work \citep{Yiyun23}.
% not trivial due to the difficulty in computing the loss function $\utilitylossT$ described in Equation~\eqref{eq:lossmeasure}.
We again consider the setting in Corollary~\ref{cor:rates} where the
underlying space $T=[0,1]^d$ is the hypercube equipped with the
$\ell_{\infty}$-metric and $T_{(i)} = [0,1]^s$ from
Theorem~\ref{thm:mainthm} are the $s$-sparse marginal subspaces.  A
straight forward instantiation of Algorithm~\ref{alg:mainalgo} in
Theorem~\ref{thm:mainthm} yields the ``slow'' run-time complexity of
order $\text{poly}(k^d,n)$ for $t=1/2k$, and in fact,  computational
hardness results \citep{dwork2009complexity,ullman2011pcps} suggest
that the exponential dependency in $d$ cannot be avoided.  
 
However, we note that the computationally hard part arises from
solving the optimization problem $\utilitylossT(\nudp, \mathbb T \mu)$
(Step 3 in Algorithm~\ref{alg:mainalgo}), while computing $\mathbb T
\mu_D$  (Step~1 in Algorithm~\ref{alg:mainalgo}) can be done in
run-time complexity of order at most $\text{poly}(d^s k^s,\vert D\vert
)$  and computing $\nudp$ (Step 2 in Algorithm~\ref{alg:mainalgo}) can
be done in run-time of the order $\text{poly}(d^s k^s)$. This
motivates the development of greedy algorithms which release a data
set $D'$ by approximately minimizing the loss function
$\utilitylossT(\nudp, \mathbb T \mu_{D'})$, where single evaluations
of this term can be performed in run-time complexity of order at most
$\text{poly}(d^s k^s,\vert D'\vert )$.  Even though the found solution
might be far from optimal,  we can guarantee that the measure
$\mu_{D'}$ is $\epsilon$-DP (respectively $(\epsilon,\delta)$-DP; see
Appendix~\ref{apx:almostsure}) and by
Equation~\eqref{eq:utilityUBgeneral} has a utility loss at most
 \begin{equation}
     \utilityloss(\mu_D, \mu_{D'}) \leq \underbrace{\utilityloss(\mu_D, \mathbb T^\dagger \mathbb T \mu_D) + \utilitylossT(\mathbb T \mu_D,\nudp)}_{ \leq\text{loss for exact algorithm}} + \utilitylossT(\nudp, \mathbb T\mu_{D'}),
 \end{equation}
 where we obtain an almost sure upper bound on the loss for the exact algorithm from Theorem~\ref{thm:asbounds} in Appendix~\ref{apx:almostsure} and an upper bound in expectation from Theorem~\ref{thm:mainthm} in Section~\ref{sec:mainthm}. 

 \subsubsection*{Acknowledgments}
K.D.\ is supported by the ETH AI Center and the ETH Foundations of
Data Science. A.S. is supported by the ETH AI Center. We would further
like to thank Afonso Bandeira for insightful discussions.

 % We refer to Appendix~\ref{apx:experiments} for numerical simulations illustrating this upper bound.

 
 
 
 % in $\text{poly}(d^s k^s)$ run-time complexity for any $v \in \mathbb 
 % R^\Tdim$. 
 
 
 % In particular, let $\mu_{D'}$ be the empirical measure of any data set $D' \in T_k^m$ with $m$ some integer (where $T_k$ are the centers of the $1/2k$-covering of $T$) found via running a greedy algorithm minimizing 
 % $\utilitylossT(\nudp, \mathbb T \mu_{D'})$ in polynomial run time.
 %We present numerical simulations in Appendix~\ref{apx:experiments}. 

 
 
 
 

 
 
 
 
 
 % We therefore motivate future research on greedy algorithms which efficiently find solutions $D' \in T^m$ (with $m = O(\text{poly}(n))$ approximately minimizing $\utilitylossT(\nudp, \mathbb T \mu_{D'})$.

 
 
 % --- the computational ``hardness'' lies in finding a measure such that $\mathbb T \mu = v$ is an optimal solution. 
 
 
 
 

 
 
 
 % The only compuational ``hard'' part is to optimize 


% Implementing the instantiation of Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthmmeasure} is not trivial due to the difficulty in computing the loss function $\utilitylossT$. We therefore focus in this discussion on the instantiation of Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthm} which has the ``slow'' run-time complexity of order $\text{poly}(k^d,n)$ 
%  when $t=1/2k$  and $T=[0,1]^d$ is the hypercube equipped with the $\ell_{\infty}$-metric.



 
 


 

% The instantiation of Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthm} is not efficient in the sense that the  
% In this last section we discuss the efficient implementations which 
% for the Algorithm~\ref{alg:mainalgo} in Theorem~\ref{thm:mainthm} when being instantiated on the hypercube




% aspects of the our main results and motivate future work. 


% When again considering the case where $t=[0,1]^d$ is the hypercube and equipped with the $\ell_{\infty}$ metric, it is not difficult to see that the algorithms in Theorem~\ref{thm:march} and \ref{thm:mainthm} have a run-time complexity of $O(\text{poly}(k^d,n))$ where we discretize the hypercube into $k^d$ $\ell_{\infty}$ balls and thus $t=1/2k$. Furthermore, implementing the algorithm in Theorem~\ref{thm:mainthmmeasure} is non-trivial and its run time unclear. 






% \subsection{Open problems:}\red{Amartya:this should probably merge with conclusion}
% We motivate two open problems resulting from this paper for future work. 
% The first problem concerns tight bounds: We provide in Corollary~\ref{cr:lowerbound} in Appendix~\ref{apx:lowerbound} a lower bound for the worst case measure $\mu_D$ of order $ \mathbb E \utilityloss (\mu_D, \algoD) \gtrsim_s  \left( \frac{d\log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}$. This shows that our upper bound in Corollary~\ref{cor:rates} is tight in $n$ up to logarithmic factors but not in $d$. Closing this gap is a challenging task for future research as we believe that novel proof ideas are necessary. 

% Furthermore, as a second problem we motivate the development of  greedy algorithms for solving the optimization problem in Equation~\eqref{eq:heuristics} without using public data and polynomial run-time algorithms which provide approximate guarantees for an approximate version of the utility loss $\utilityloss$. 













% we can simply add and substract constants





% However, when $\mathcal F$ is the set of all $1$-Lipschitz continuous functions we have $\tilde  \utilitylossT(v, v') = \infty$ if $\|v\|_1 \neq \|v'\|$, making such a loss function infeasible. 


% First note that we can assume without loss of generality that $\mathcal F$





% We again first state the proof of Corollary~\ref{cor:ratesmeasure} and the present in Section~\ref{subsec:proofmeasure} the proof of the theorem. 
% \paragraph{Proof of Corollary~\ref{cor:ratesmeasure}}











% This result can be understood as an adaptivity statement for releasing private measures. 



% % Our result stands in analogy to adaptivity results for the prediction error in machine learning.













% We first present in Section~\ref{subsec:numerical} numerical simulations illustrating the upper bound in Theorem~\ref{thm:mainthm}, followed by a discuss of directions for practically efficient implementations in Section~\ref{sec:practical}
% \subsection{Numerical simulations}
% \label{subsec:numerical}

% The content in this section is:
% \begin{enumerate}
%     \item When instantiating the upper bound (we can even tighten the uppper bound) we obtain 
%     ....
%     \item we now compare this with the actul wasserstein distance of the loss
% \end{enumerate}



% \subsection{Practical aspects}
% \label{subsec:practical}


% Although Corollary~\ref{cor:rates} allows to overcome the course of dimensionality when choosing $s$ small, implementations of Algorithm~\ref{alg:mainalgo} have run-time complexity $\text{poly}(k^d)$ with $k = \frac{1}{2t}$. 




% \begin{enumerate}
%     \item When instantiating the upper bound (we can even tighten the uppper bound) we obtain 
%     ....
%     \item we now compare this with the actul wasserstein distance of the loss
% \end{enumerate}























   





% We now discuss the case where the dataset $T \subset \mathbb R^d$ is a compact subset of $\mathbb R^d$ and the goal is to construct an DP algorithm which achieves high utility on sparse Lipschitz continuous functions. 
% \red{Say something about the importance of this problem}


% In this section, we do bla bla


% For simplicity, for the following discussion we choose $T = [0,1]^d$ to be the $d$-dimensional hypercube and let $\mathcal F$ be the set of $s$-sparse Lispchitz continuous functions (i.e. $f$ only depends on $s$-dimensions),
% \begin{equation}
%     \mathcal F_s := \{f\vert~ f~1\text{-Lipschitz~w.r.t. }\|.\|_{\infty}\text{-norm~and~} f~\text{is}~s\text{-sparse}\}.
% \end{equation}
% To obtain an upper bound for the utility loss, we can apply Theorem~\ref{thm:mainthm} which yields the following corollary when using that $K ={d \choose s}$, 
% \begin{equation}
% N(T_{(i)}, \|.\|_{\infty},t) \leq (1/t)^s
% \end{equation}
%  and after optimizing over $t$:
% \begin{corollary}
% For any $n,d$ sufficiently large with $n\epsilon \geq d$ and constant $s$,  
% there exists an $\epsilon$-DP algorithm such that
% \begin{equation}
% \label{eq:ubfull}
%     \mathbb E U_{\mathcal F_s}(\mu_D, \algoD) \lesssim \sqrt{d} \left( \frac{\log(\epsilon n)^{3/2}}{n \epsilon}\right)^{1/s}.
% \end{equation}
% Furthermore, there exists an $(\epsilon,\delta)$-DP algorithm such that almost surely, 
% \begin{equation}
% \label{eq:ubfull}
%      U_{\mathcal F_s}(\mu_D, \algoD) \lesssim \sqrt{d} \left( \frac{\log(\epsilon n)^{2} \log(1 + \frac{e^\epsilon -1}{2 \delta})}{n \epsilon}\right)^{1/s}.
% \end{equation}
% \end{corollary}





% This bound is tight up to log factors, as we obtain a lower bound of order



% \begin{proposition}
% Lower bound
% \begin{equation}
%     \mathbb E W_1(\mu, v) \gtrsim \sqrt{d} \left( \frac{1}{n \epsilon}\right)^{1/s}.
% \end{equation}
% \end{proposition}


% \subsection{Efficient algorithms}





% \subsection{Numerical experiments}








% metrically private Algorithms. By  an algorithm $\mathcal A: \measure_0 \to \measure_1$ is $\epsilon$-DP if and only if $\mathcal A$ is $\epsilon n$-metrically private with respect to the normalized Hamming distance $\rho_1$. That is, for all measures $\mu_D, \mu_{D'} \in \measure_0$ and any subset of measures $V \subset \measure_1$ we have that
% \begin{align}
%     \frac{\mathbb P( \algoD \in V)}{\mathbb P( \mathcal A(\mu_{D'}) \in V)}\leq \exp\left(\epsilon n \rho_0(\mu_D, \mu_{D'})\right).
% \end{align}


==> sections/old_text.tex <==
While the algorithm in Section~\ref{subsec:algo} comes with theoretical guarantees for the decay rate of the utility loss (see
Section~\ref{sec:mainthm}), in many practical applications we prefer actual upper bounds on the utility loss for a specific setting.


We now describe how we can obtain a plug-in type upper bound for the utility loss \ref{eq:utilityloss}.  We  assume that  $\mathbb T$ is as described in Section~\ref{subsec:algo} and that $\nudp$ in Step 2 of Algorithm~\ref{alg:mainalgo} is generated using the Laplace mechanism  in Equation~\eqref{eq:noiseeq} with $\Phi$ any matrix (or any similar mechanism such as the Guassian or discrete Laplace mechanism). The idea is now to define the loss $ \utilityloss_{\mathbb T}: \mathbb R^m \times \mathbb R^m \to \mathbb R_+$ such that
for any two measures $\mu, \mu' \in \mathcal M(T)$:
\begin{equation}\label{eq:uequt}
    \mathcal U(\mathbb T^\dagger \mathbb T \mu, \mathbb T^\dagger \mathbb T \mu') = \utilityloss_{\mathbb T}(\mathbb T\mu, \mathbb T \mu'). 
\end{equation}
 By the choice of $\mathbb T$ (see Section~\ref{subsec:algo}), for any vector $u \in \mathbb R^m$, any block $u^{(j)}$ of  $u$  represents a  discrete signed measure  on the $s$-dimensional discrete hyper cube $T_{k,s} := \{ 1/2k, \cdots , (2k-1)/2k\}^s$, which we denote with $\omega^{(j)}_{u} := \underset{z_i \in T_{k,s}}{\sum}\delta[z_i]\left(u^{(j)}\right)_i$. It is now an straight forward task to verify that the following definition for $\utilityloss_{\mathbb T}$ indeed satisfies the equality in Equation~\eqref{eq:uequt}:
\begin{equation}
\label{eq:lossmeasure}
 \utilityloss_{\mathbb T}(v, u) :=  \max_{j \in \left\{1, \cdots, {d \choose s}\right\} } \sup_{\substack{f \in \mathcal F(T_{k,s})\\ \|f \|_{\infty} \leq 1}} \left \vert \sum_{z_i \in T_{k,s}} f(z_i) ~ \omega^{(j)}_{v}(\{z_i\}) - \sum_{z_i \in T_\Tdim} f(z_i) ~\omega^{(j)}_{u}(\{z_i\})\right \vert, 
\end{equation}
where $\mathcal F(T_{k,s})$ is the set of all $1$-Lipschitz continuous functions  over $T_{k,s}$ w.r.t.~the $\ell_\infty$-distance function. In particular, the RHS in Equation~\eqref{eq:lossmeasure} can be efficiently computed by taking the maximum over $C(d, s)$ solutions of linear programs, with a run-time complexity of 
$O\left(C(d, s) \text{poly}(k^s) \right)$.




% where $\mathcal F_{S_j}$ is the set of $1$-Lipschitz continuous functions which only depend on the indices in $S_j$ and $M^\dagger_j$ the pseudo inverse of $M_j$. Note that the vector $ M_j^\dagger v^{(j)}$ represents a (discrete) measure on $\mathcal M(T_k) \subset \mathcal M(T)$, and thus with a slight abuse of notation, we write 
% $( M_j^\dagger v^{(j)})(\{z_i\})$ for the mass of $z_i \in T_k$. 
% The loss $\utilityloss_{\mathbb T}$ can be understood as an extension of the utility loss for the operator $\mathbb T$ since
% for any two measures $\mu, \mu' \in \mathcal M(T)$:
% \begin{equation}\label{eq:yizheloss}
%     \mathcal U(\mathbb T^\dagger \mathbb T \mu, \mathbb T^\dagger \mathbb T \mu') = \utilityloss_{\mathbb T}(\mathbb T\mu, \mathbb T \mu'). 
% \end{equation}


We can now simultaneously upper bound for any discrete measure $\tilde \mu \in \mathcal M(T_k) \subset \mathcal M(T)$ the utility loss by:
\begin{equation}
    \begin{split}
   \utilityloss(\mu_D, \tilde \mu) 
   &\leq \utilityloss(\mu_D,\mathbb T ^\dagger\mathbb T\mu_D)+\utilityloss(\mathbb T^\dagger\mathbb T\mu_D,\mathbb T^\dagger \mathbb T \tilde \mu )+\utilityloss(\tilde \mu,\mathbb T^\dagger\mathbb T\tilde \mu)
   \\
   &=
   \utilityloss(\mu_D,\mathbb T ^\dagger\mathbb T\mu_D)+\utilityloss_{\mathbb T}(\mathbb T\mu_D,\mathbb T\tilde \mu )\\
   &\leq
   \utilityloss(\mu_D,\mathbb T ^\dagger\mathbb T\mu_D)+\utilityloss_{\mathbb T}(\mathbb T\mu_D,\nudp) + \utilityloss_{\mathbb T}(\nudp, \mathbb T\tilde \mu)
   \label{eq:ubsec23}
   \end{split}
\end{equation}

where in the second line we used that $  \utilityloss(\tilde \mu,\mathbb T^\dagger\mathbb T\tilde \mu) =0$. In particular,  $\utilityloss(\mu_D,\mathbb T ^\dagger\mathbb T\mu_D) \leq 1/2k$ since $T_k$ is a $1/2k$ covering of $T$. Furthermore, we note that the term $\utilityloss_{\mathbb T}(\mathbb T \mu_D , \nudp)$ does not depend on $D$ but only on the noise $\eta$ form Equation~\eqref{eq:noiseeq}:
\begin{equation}
\label{eq:onlynoise}    \utilityloss_{\mathbb T}(\mathbb T \mu_D , \nudp) = \utilityloss_{\mathbb T}(\mathbb T \mu_D  - \nudp, 0) = \utilityloss_{\mathbb T}(\left[\Phi \eta \right]_{1:\Tdim}, 0).
\end{equation}

Thus, for any $\delta >0$ we can approximate the $1-\delta$-quantile $q_{1-\delta, \mathbb T} := q_{1-\delta}(\utilityloss_{\mathbb T}(\left[\Phi \eta \right]_{1:\Tdim}, 0))$. Finally, since $\nudp$ is a DP-vector, we can simply compute the third term in Equation~\eqref{eq:onlynoise}. Hence, we obtain the upper bound on the utility loss which holds with probability at least $1-\delta$ over the draws of the noise $\eta$:
\begin{equation}
        \utilityloss(\mu_D, \tilde \mu) \leq \underbrace{\frac{1}{2k} + q_{1-\delta, \mathbb T}}_{\text{constant term}} + \utilityloss_{\mathbb T}(\nudp, \mathbb T\tilde \mu), \label{eq:ub}
\end{equation}
